An Updated Experimental Evaluation of Graph Bipartization Methods

We experimentally evaluate the practical state-of-the-art in graph bipartization (Odd Cycle Transversal), motivated by recent advances in near-term quantum computing hardware and the related embedding problems. We assemble a preprocessing suite of fast input reduction routines from the Odd Cycle Transversal (OCT) and Vertex Cover (VC) literature, and compare algorithm implementations using Quadratic Unconstrained Binary Optimization problems from the quantum literature. We also generate a corpus of frustrated cluster loop graphs, which have previously been used to benchmark quantum annealing hardware. The diversity of these graphs leads to harder OCT instances than in existing benchmarks. In addition to combinatorial branching algorithms for solving OCT directly, we study various reformulations into other NP-hard problems such as VC and Integer Linear Programming (ILP), enabling the use of solvers such as CPLEX. We find that for heuristic solutions with time constraints under a second, iterative compression routines jump-started with a heuristic solution perform best, after which point using a highly tuned solver like CPLEX is worthwhile. Results on exact solvers are split between using ILP formulations on CPLEX and solving VC formulations with a branch-and-reduce solver. We extend our results with a large corpus of synthetic graphs, establishing robustness and potential to generalize to other domain data. In total, over 8000 graph instances are evaluated, compared to the previous canonical corpus of 100 graphs. Finally, we provide all code and data in an open source suite, including a Python API for accessing reduction routines and branching algorithms, along with scripts for fully replicating our results.

==> tables/exact_full.tex <==
\begin{tabular}{lrrrrp{0.5in}lrrrr}
\toprule
  \multicolumn{2}{c}{\textbf{Graph}}            & \multicolumn{3}{c}{\textbf{Solver}}            &            & \multicolumn{2}{c}{\textbf{Graph}}            & \multicolumn{3}{c}{\textbf{Solver}} \\
\cmidrule(lr){1-2}
\cmidrule(lr){3-5}
\cmidrule(lr){7-8}
\cmidrule(lr){9-11}
\textbf{Dataset} & $OPT'$ & \textsf{VC} & \textsf{IC} & \textsf{ILP} & & \textbf{Dataset} & $OPT'$ & \textsf{VC} & \textsf{IC} & \textsf{ILP} \\
\midrule
\texttt{aa-10} & 6 & 0.2 & 1.0 & 0.0 & & \texttt{j-25} & 0 & 0.1 & 1.0 & 0.0 \\
\texttt{aa-11} & 11 & 0.1 & 1.0 & 0.1 & & \texttt{j-26} & 6 & 0.1 & 1.0 & 0.0 \\
\texttt{aa-13} & 12 & 0.1 & 1.0 & 0.1 & & \texttt{j-28} & 13 & 0.1 & 1.0 & 0.0 \\
\texttt{aa-14} & 19 & 0.2 & 4.7 & 0.1 & & \texttt{b-50-1} & 11 & 0.1 & 1.0 & 0.1 \\
\texttt{aa-15} & 6 & 0.1 & 1.0 & 0.0 & & \texttt{b-50-2} & 11 & 0.1 & 1.0 & 0.0 \\
\texttt{aa-16} & 0 & 0.1 & 1.0 & 0.0 & & \texttt{b-50-3} & 14 & 0.2 & 1.2 & 0.0 \\
\texttt{aa-17} & 25 & 0.4 & 6.4 & 0.1 & & \texttt{b-50-4} & 11 & 0.1 & 1.0 & 0.0 \\
\texttt{aa-18} & 14 & 0.1 & 1.0 & 0.0 & & \texttt{b-50-5} & 13 & 0.2 & 1.1 & 0.1 \\
\texttt{aa-19} & 19 & 0.2 & 2.7 & 0.2 & & \texttt{b-50-6} & 9 & 0.1 & 1.0 & 0.0 \\
\texttt{aa-20} & 19 & 0.3 & 1.1 & 0.1 & & \texttt{b-50-7} & 9 & 0.1 & 1.0 & 0.0 \\
\texttt{aa-21} & 0 & 0.1 & 1.0 & 0.0 & & \texttt{b-50-8} & 14 & 0.2 & 1.4 & 0.1 \\
\texttt{aa-22} & 16 & 0.2 & 1.0 & 0.1 & & \texttt{b-50-9} & 12 & 0.2 & 1.1 & 0.1 \\
\texttt{aa-23} & 18 & 0.2 & 1.0 & 0.1 & & \texttt{b-50-10} & 11 & 0.1 & 1.0 & 0.1 \\
\texttt{aa-24} & 21 & 0.3 & 1.4 & 0.1 & & \texttt{b-100-1} & 41 & 97.8 & - & 21.3 \\
\texttt{aa-25} & 0 & 0.1 & 1.0 & 0.0 & & \texttt{b-100-2} & 42 & 185.5 & - & 52.7 \\
\texttt{aa-26} & 12 & 0.1 & 1.0 & 0.0 & & \texttt{b-100-3} & 42 & 242.3 & - & 20.9 \\
\texttt{aa-27} & 11 & 0.2 & 1.0 & 0.1 & & \texttt{b-100-4} & 41 & 199.8 & - & 33.1 \\
\texttt{aa-28} & 27 & 0.2 & 1.1 & 0.1 & & \texttt{b-100-5} & 42 & 208.6 & - & 41.7 \\
\texttt{aa-29} & 21 & 0.3 & 1.1 & 0.1 & & \texttt{b-100-6} & 43 & 143.6 & - & 99.6 \\
\texttt{aa-30} & 4 & 0.1 & 1.0 & 0.0 & & \texttt{b-100-7} & 42 & 182.0 & - & 40.4 \\
\texttt{aa-31} & 0 & 0.1 & 1.0 & 0.0 & & \texttt{b-100-8} & 43 & 356.7 & - & 39.3 \\
\texttt{aa-32} & 30 & 0.6 & 10.2 & 0.5 & & \texttt{b-100-9} & 44 & 321.4 & - & 72.9 \\
\texttt{aa-33} & 4 & 0.1 & 1.0 & 0.0 & & \texttt{b-100-10} & 44 & 188.6 & - & 118.3 \\
\texttt{aa-34} & 13 & 0.2 & 1.0 & 0.1 & & \texttt{gka-1} & 9 & 0.1 & 1.0 & 0.1 \\
\texttt{aa-35} & 10 & 0.1 & 1.0 & 0.0 & & \texttt{gka-2} & 16 & 0.4 & 2.2 & 0.1 \\
\texttt{aa-36} & 7 & 0.1 & 1.0 & 0.0 & & \texttt{gka-3} & 23 & 1.4 & 58.0 & 0.9 \\
\texttt{aa-37} & 4 & 0.1 & 1.0 & 0.0 & & \texttt{gka-4} & 28 & 4.4 & - & 2.3 \\
\texttt{aa-38} & 26 & 0.3 & 1.5 & 0.1 & & \texttt{gka-5} & 22 & 0.7 & 3.4 & 0.1 \\
\texttt{aa-39} & 23 & 0.3 & 2.7 & 0.1 & & \texttt{gka-6} & 16 & 0.1 & 1.0 & 0.1 \\
\texttt{aa-40} & 22 & 0.3 & 1.5 & 0.1 & & \texttt{gka-7} & 18 & 0.1 & 1.0 & 0.0 \\
\texttt{aa-41} & 40 & 0.8 & 48.0 & 0.4 & & \texttt{gka-8} & 28 & 7.2 & - & 4.8 \\
\texttt{aa-42} & 30 & 0.4 & 2.1 & 0.3 & & \texttt{gka-9} & 2 & 0.1 & 1.0 & 0.0 \\
\texttt{aa-43} & 18 & 0.1 & 1.0 & 0.1 & & \texttt{gka-10} & 8 & 0.1 & 1.0 & 0.0 \\
\texttt{aa-44} & 10 & 0.1 & 1.0 & 0.0 & & \texttt{gka-11} & 10 & 0.1 & 1.0 & 0.0 \\
\texttt{aa-45} & 20 & 0.2 & 1.1 & 0.1 & & \texttt{gka-12} & 20 & 0.1 & 1.0 & 0.0 \\
\texttt{aa-46} & 13 & 0.2 & 1.0 & 0.1 & & \texttt{gka-13} & 16 & 0.1 & 1.0 & 0.0 \\
\texttt{aa-47} & 13 & 0.1 & 1.0 & 0.0 & & \texttt{gka-14} & 22 & 0.1 & 1.0 & 0.0 \\
\texttt{aa-48} & 17 & 0.1 & 1.0 & 0.1 & & \texttt{gka-15} & 0 & 0.1 & 1.0 & 0.0 \\
\texttt{aa-49} & 0 & 0.1 & 1.0 & 0.0 & & \texttt{gka-16} & 0 & 0.1 & 1.0 & 0.0 \\
\texttt{aa-50} & 18 & 0.2 & 1.0 & 0.1 & & \texttt{gka-17} & 0 & 0.1 & 1.0 & 0.0 \\
\texttt{aa-51} & 11 & 0.1 & 1.0 & 0.0 & & \texttt{gka-18} & 2 & 0.1 & 1.0 & 0.0 \\
\texttt{aa-52} & 12 & 0.1 & 1.0 & 0.1 & & \texttt{gka-19} & 31 & 0.2 & 1.0 & 0.1 \\
\texttt{aa-53} & 12 & 0.1 & 1.0 & 0.1 & & \texttt{gka-20} & 39 & 0.6 & 1.2 & 0.1 \\
\texttt{aa-54} & 12 & 0.2 & 1.0 & 0.1 & & \texttt{gka-21} & 40 & 1.7 & 22.2 & 0.3 \\
\texttt{j-10} & 3 & 0.1 & 1.0 & 0.0 & & \texttt{gka-22} & 43 & 5.4 & - & 1.0 \\
\texttt{j-11} & 5 & 0.1 & 1.0 & 0.0 & & \texttt{gka-23} & 46 & 42.6 & - & 16.9 \\
\texttt{j-13} & 4 & 0.1 & 1.0 & 0.0 & & \texttt{gka-24} & 37 & 74.3 & - & 17.3 \\
\texttt{j-14} & 3 & 0.1 & 1.0 & 0.0 & & \texttt{gka-25} & 42 & 122.9 & - & 28.6 \\
\texttt{j-15} & 0 & 0.1 & 1.0 & 0.0 & & \texttt{gka-26} & 43 & 160.5 & - & 18.4 \\
\texttt{j-16} & 0 & 0.1 & 1.0 & 0.0 & & \texttt{gka-27} & 62 & 535.3 & - & 192.6 \\
\texttt{j-17} & 10 & 0.1 & 1.0 & 0.0 & & \texttt{gka-28} & 70 & 284.9 & - & 366.0 \\
\texttt{j-18} & 9 & 0.1 & 1.0 & 0.0 & & \texttt{gka-29} & 77 & 64.3 & - & 42.5 \\
\texttt{j-19} & 3 & 0.1 & 1.0 & 0.0 & & \texttt{gka-30} & 82 & 32.7 & - & 53.2 \\
\texttt{j-20} & 0 & 0.1 & 1.0 & 0.0 & & \texttt{gka-31} & 85 & 11.7 & 107.6 & 17.4 \\
\texttt{j-21} & 2 & 0.1 & 1.0 & 0.0 & & \texttt{gka-32} & 88 & 5.3 & 17.9 & 19.2 \\
\texttt{j-22} & 9 & 0.1 & 1.0 & 0.0 & & \texttt{gka-33} & 90 & 4.0 & 3.1 & 2.2 \\
\texttt{j-23} & 19 & 0.1 & 1.1 & 0.1 & & \texttt{gka-34} & 92 & 2.5 & 1.2 & 1.4 \\
\texttt{j-24} & 3 & 0.1 & 1.0 & 0.0 & & \texttt{gka-35} & 0 & 0.1 & 1.0 & 0.0 \\
\bottomrule
\end{tabular}


==> tables/generated_preprocessed_full.tex <==
\begin{tabular}{lrrrrrrrrrr}
\toprule
  Dataset &  $|V|$ &  $|E|$ &  $OPT$ &  $|V_r|$ &  $|E_r|$ &  $|V_o|$ &  $|V_b|$ &  $|V' \cup V_b|$ &  $|E'|$ &  $OPT'$ \\
\midrule
    aa-10 &     69 &    191 &      6 &       10 &        0 &        0 &       30 &               59 &     181 &       6 \\
    aa-11 &    103 &    307 &     11 &       10 &        0 &        0 &       62 &               93 &     298 &      11 \\
    aa-13 &    131 &    383 &     12 &       10 &        0 &        0 &       79 &              121 &     375 &      12 \\
    aa-14 &    127 &    525 &     19 &       16 &        0 &        0 &       66 &              111 &     512 &      19 \\
    aa-15 &     67 &    179 &      7 &       15 &        0 &        1 &       21 &               51 &     146 &       6 \\
    aa-16 &     14 &     15 &      0 &       14 &        0 &        0 &        0 &                0 &       0 &       0 \\
    aa-17 &    153 &    633 &     25 &        7 &        0 &        0 &       91 &              146 &     628 &      25 \\
    aa-18 &     90 &    381 &     14 &       11 &        0 &        0 &       33 &               79 &     373 &      14 \\
    aa-19 &    192 &    645 &     19 &       11 &        0 &        0 &      120 &              181 &     636 &      19 \\
    aa-20 &    225 &    766 &     19 &        7 &        0 &        0 &      161 &              218 &     760 &      19 \\
    aa-21 &     31 &     90 &      9 &       22 &        0 &        9 &        0 &                0 &       0 &       0 \\
    aa-22 &    167 &    641 &     16 &        5 &        0 &        0 &      115 &              162 &     636 &      16 \\
    aa-23 &    143 &    508 &     18 &       21 &        0 &        0 &       69 &              122 &     492 &      18 \\
    aa-24 &    261 &   1108 &     21 &       12 &        0 &        0 &      169 &              249 &    1099 &      21 \\
    aa-25 &     15 &     15 &      1 &       14 &        0 &        1 &        0 &                0 &       0 &       0 \\
    aa-26 &     95 &    284 &     13 &       21 &        0 &        1 &       33 &               73 &     255 &      12 \\
    aa-27 &    120 &    331 &     11 &       12 &        0 &        0 &       61 &              108 &     322 &      11 \\
    aa-28 &    167 &    854 &     27 &       13 &        0 &        0 &       89 &              154 &     841 &      27 \\
    aa-29 &    277 &   1058 &     21 &       12 &        0 &        0 &      197 &              265 &    1048 &      21 \\
    aa-30 &     39 &     71 &      4 &        9 &        0 &        0 &       12 &               30 &      61 &       4 \\
    aa-31 &     30 &     51 &      2 &       28 &        0 &        2 &        0 &                0 &       0 &       0 \\
    aa-32 &    151 &    750 &     30 &       25 &        0 &        0 &       61 &              126 &     733 &      30 \\
    aa-33 &    194 &    493 &      4 &       12 &        0 &        0 &      143 &              182 &     481 &       4 \\
    aa-34 &    134 &    451 &     13 &       12 &        0 &        0 &       85 &              122 &     440 &      13 \\
    aa-35 &     82 &    269 &     10 &        6 &        0 &        0 &       38 &               76 &     264 &      10 \\
    aa-36 &    112 &    316 &      7 &        9 &        0 &        0 &       68 &              103 &     309 &       7 \\
    aa-37 &     73 &    170 &      5 &       24 &        0 &        1 &       22 &               49 &     120 &       4 \\
    aa-38 &    171 &    862 &     26 &       10 &        0 &        0 &       94 &              161 &     852 &      26 \\
    aa-39 &    145 &    692 &     23 &        4 &        0 &        0 &       82 &              141 &     689 &      23 \\
    aa-40 &    140 &    620 &     22 &       20 &        0 &        0 &       60 &              120 &     604 &      22 \\
    aa-41 &    300 &   1620 &     40 &       39 &        0 &        0 &      172 &              261 &    1585 &      40 \\
    aa-42 &    237 &   1110 &     30 &       11 &        0 &        0 &      137 &              226 &    1100 &      30 \\
    aa-43 &     64 &    308 &     18 &        6 &        0 &        0 &       18 &               58 &     303 &      18 \\
    aa-44 &     60 &    163 &     10 &        7 &        0 &        0 &       23 &               53 &     157 &      10 \\
    aa-45 &     83 &    386 &     20 &        8 &        0 &        0 &       32 &               75 &     381 &      20 \\
    aa-46 &    163 &    529 &     13 &       17 &        0 &        0 &       89 &              146 &     514 &      13 \\
    aa-47 &     65 &    229 &     14 &       17 &        0 &        1 &       13 &               47 &     195 &      13 \\
    aa-48 &     90 &    343 &     17 &       14 &        0 &        0 &       35 &               76 &     330 &      17 \\
    aa-49 &     27 &     62 &      5 &       22 &        0 &        5 &        0 &                0 &       0 &       0 \\
    aa-50 &    113 &    468 &     18 &        5 &        0 &        0 &       48 &              108 &     463 &      18 \\
    aa-51 &     79 &    274 &     11 &        8 &        0 &        0 &       27 &               71 &     268 &      11 \\
    aa-52 &     66 &    231 &     14 &       20 &        0 &        2 &       14 &               46 &     183 &      12 \\
    aa-53 &     89 &    232 &     12 &        9 &        0 &        0 &       37 &               80 &     224 &      12 \\
    aa-54 &     90 &    233 &     12 &       13 &        0 &        0 &       31 &               77 &     222 &      12 \\
     j-10 &     57 &    117 &      3 &       20 &        0 &        0 &       13 &               37 &      97 &       3 \\
     j-11 &     51 &    212 &      5 &       14 &        0 &        0 &        8 &               37 &     198 &       5 \\
     j-13 &     78 &    210 &      6 &       22 &        0 &        2 &       28 &               54 &     153 &       4 \\
     j-14 &     72 &    107 &      4 &       52 &        0 &        1 &        3 &               19 &      55 &       3 \\
     j-15 &     45 &     55 &      1 &       44 &        0 &        1 &        0 &                0 &       0 &       0 \\
     j-16 &     14 &     10 &      0 &       14 &        0 &        0 &        0 &                0 &       0 &       0 \\
     j-17 &     81 &    322 &     10 &       20 &        0 &        0 &       20 &               61 &     304 &      10 \\
     j-18 &     73 &    296 &      9 &       15 &        0 &        0 &       11 &               58 &     284 &       9 \\
     j-19 &    101 &    172 &      3 &       63 &        0 &        0 &       20 &               38 &     116 &       3 \\
     j-20 &    241 &    640 &      1 &      240 &        0 &        1 &        0 &                0 &       0 &       0 \\
     j-21 &     33 &    102 &      9 &       18 &        0 &        7 &        1 &                8 &      16 &       2 \\
     j-22 &     76 &    391 &      9 &        9 &        0 &        0 &       23 &               67 &     384 &       9 \\
     j-23 &     76 &    369 &     19 &       25 &        0 &        0 &        1 &               51 &     345 &      19 \\
     j-24 &    150 &    387 &      4 &       83 &        0 &        1 &       20 &               66 &     265 &       3 \\
     j-25 &     14 &     14 &      0 &       14 &        0 &        0 &        0 &                0 &       0 &       0 \\
     j-26 &     65 &    156 &      6 &       29 &        0 &        0 &       10 &               37 &     126 &       6 \\
     j-28 &     96 &    567 &     13 &       22 &        0 &        0 &       17 &               74 &     552 &      13 \\
    gka-1 &     50 &    106 &     10 &        4 &        0 &        2 &        9 &               44 &      90 &       9 \\
    gka-2 &     60 &    163 &     17 &        1 &        0 &        1 &        1 &               58 &     149 &      16 \\
    gka-3 &     70 &    223 &     23 &        0 &        0 &        0 &        4 &               70 &     223 &      23 \\
    gka-4 &     80 &    304 &     28 &        0 &        0 &        0 &        0 &               80 &     304 &      28 \\
    gka-5 &     50 &    231 &     22 &        0 &        0 &        0 &        0 &               50 &     231 &      22 \\
    gka-6 &     30 &    174 &     16 &        0 &        0 &        0 &        0 &               30 &     174 &      16 \\
    gka-7 &     30 &    211 &     18 &        0 &        0 &        0 &        0 &               30 &     211 &      18 \\
    gka-8 &    100 &    304 &     28 &        1 &        0 &        0 &        5 &               99 &     303 &      28 \\
    gka-9 &     20 &    187 &     16 &        0 &        0 &       14 &        0 &                6 &      12 &       2 \\
   gka-10 &     30 &    429 &     26 &        0 &        0 &       18 &        0 &               12 &      60 &       8 \\
   gka-11 &     40 &    772 &     36 &        0 &        0 &       26 &        0 &               14 &      84 &      10 \\
   gka-12 &     50 &   1209 &     46 &        0 &        0 &       26 &        0 &               24 &     264 &      20 \\
   gka-13 &     60 &   1751 &     56 &        0 &        0 &       40 &        0 &               20 &     180 &      16 \\
   gka-14 &     70 &   2388 &     66 &        0 &        0 &       44 &        0 &               26 &     312 &      22 \\
   gka-15 &     80 &   3125 &     76 &        4 &        0 &       76 &        0 &                0 &       0 &       0 \\
   gka-16 &     90 &   3963 &     86 &        4 &        0 &       86 &        0 &                0 &       0 &       0 \\
   gka-17 &    100 &   4903 &     96 &        4 &        0 &       96 &        0 &                0 &       0 &       0 \\
   gka-18 &    125 &   7666 &    120 &        0 &        0 &      118 &        1 &                7 &      16 &       2 \\
   gka-19 &     40 &    625 &     32 &        0 &        0 &        1 &        0 &               39 &     588 &      31 \\
   gka-20 &     50 &    763 &     39 &        0 &        0 &        0 &        0 &               50 &     763 &      39 \\
   gka-21 &     60 &    701 &     40 &        0 &        0 &        0 &        0 &               60 &     701 &      40 \\
   gka-22 &     70 &    720 &     43 &        0 &        0 &        0 &        0 &               70 &     720 &      43 \\
   gka-23 &     80 &    641 &     46 &        0 &        0 &        0 &        0 &               80 &     641 &      46 \\
   gka-24 &     90 &    400 &     37 &        0 &        0 &        0 &        0 &               90 &     400 &      37 \\
   gka-25 &    100 &    495 &     42 &        0 &        0 &        0 &        1 &              100 &     495 &      42 \\
   gka-26 &    100 &    494 &     43 &        0 &        0 &        0 &        0 &              100 &     494 &      43 \\
   gka-27 &    100 &   1016 &     62 &        0 &        0 &        0 &        0 &              100 &    1016 &      62 \\
   gka-28 &    100 &   1425 &     70 &        0 &        0 &        0 &        0 &              100 &    1425 &      70 \\
   gka-29 &    100 &   2000 &     77 &        0 &        0 &        0 &        0 &              100 &    2000 &      77 \\
   gka-30 &    100 &   2414 &     82 &        0 &        0 &        0 &        0 &              100 &    2414 &      82 \\
   gka-31 &    100 &   2948 &     85 &        0 &        0 &        0 &        0 &              100 &    2948 &      85 \\
   gka-32 &    100 &   3434 &     88 &        0 &        0 &        0 &        0 &              100 &    3434 &      88 \\
   gka-33 &    100 &   3907 &     90 &        0 &        0 &        0 &        0 &              100 &    3907 &      90 \\
   gka-34 &    100 &   4346 &     92 &        0 &        0 &        0 &        0 &              100 &    4346 &      92 \\
   gka-35 &    100 &   4897 &     96 &        4 &        0 &       96 &        0 &                0 &       0 &       0 \\
   b-50-1 &     50 &    108 &     11 &        0 &        0 &        0 &        5 &               50 &     108 &      11 \\
   b-50-2 &     50 &    120 &     11 &        3 &        0 &        0 &        4 &               47 &     118 &      11 \\
   b-50-3 &     50 &    132 &     14 &        0 &        0 &        0 &        3 &               50 &     132 &      14 \\
   b-50-4 &     50 &    111 &     11 &        4 &        0 &        0 &        8 &               46 &     108 &      11 \\
   b-50-5 &     50 &    131 &     13 &        0 &        0 &        0 &        3 &               50 &     131 &      13 \\
   b-50-6 &     50 &    101 &      9 &        7 &        0 &        0 &        5 &               43 &      97 &       9 \\
   b-50-7 &     50 &    124 &     10 &        1 &        0 &        1 &        4 &               48 &     116 &       9 \\
   b-50-8 &     50 &    137 &     14 &        0 &        0 &        0 &        4 &               50 &     137 &      14 \\
   b-50-9 &     50 &    122 &     12 &        4 &        0 &        0 &        2 &               46 &     118 &      12 \\
  b-50-10 &     50 &    108 &     11 &        2 &        0 &        0 &        6 &               48 &     106 &      11 \\
  b-100-1 &    100 &    464 &     41 &        0 &        0 &        0 &        0 &              100 &     464 &      41 \\
  b-100-2 &    100 &    482 &     42 &        0 &        0 &        0 &        0 &              100 &     482 &      42 \\
  b-100-3 &    100 &    490 &     42 &        0 &        0 &        0 &        1 &              100 &     490 &      42 \\
  b-100-4 &    100 &    475 &     41 &        0 &        0 &        0 &        0 &              100 &     475 &      41 \\
  b-100-5 &    100 &    459 &     42 &        0 &        0 &        0 &        0 &              100 &     459 &      42 \\
  b-100-6 &    100 &    510 &     43 &        0 &        0 &        0 &        0 &              100 &     510 &      43 \\
  b-100-7 &    100 &    469 &     42 &        0 &        0 &        0 &        0 &              100 &     469 &      42 \\
  b-100-8 &    100 &    492 &     43 &        0 &        0 &        0 &        0 &              100 &     492 &      43 \\
  b-100-9 &    100 &    502 &     44 &        0 &        0 &        0 &        1 &              100 &     502 &      44 \\
 b-100-10 &    100 &    485 &     44 &        0 &        0 &        0 &        0 &              100 &     485 &      44 \\
\bottomrule
\end{tabular}


==> tables/generated_preprocessed_summary.tex <==
\begin{tabular}{lrrrrrrrrrr}
\toprule
Dataset & Vertex Range & Density Range &      OPT & V Removed & E Removed &   OCT & Bipartite & Remaining V Range & Remaining E Range &    OPT' \\
\midrule
     aa &      14--300 &      1.0--5.4 &    0--40 &      13\% &       0\% &   0\% &      62\% &            0--265 &          2.0--6.1 &   0--40 \\
      j &      14--241 &      0.7--5.9 &    0--19 &      41\% &       0\% &   0\% &      10\% &             0--74 &          2.0--7.5 &   0--19 \\
    gka &      20--125 &     2.1--61.3 &  10--120 &       0\% &       0\% &  18\% &       0\% &            0--100 &         2.0--43.5 &   0--92 \\
   b-50 &       50--50 &      2.0--2.7 &    9--14 &       2\% &       0\% &   0\% &       4\% &            43--50 &          2.2--2.7 &   9--14 \\
  b-100 &     100--100 &      4.6--5.1 &   41--44 &       0\% &       0\% &   0\% &       0\% &          100--100 &          4.6--5.1 &  41--44 \\
\bottomrule
\end{tabular}


==> tables/generated_preprocessed_synthetic_full.tex <==
\begin{tabular}{lrrrrrrrrrr}
\toprule
     Dataset &  original_vertices &  original_edges &  vertices_removed &  edges_removed &  oct &  bipartite &  final_vertices &  final_edges &  $|V|$ &  $|E|$ \\
\midrule
     aa10-er &                 69 &             179 &                 2 &              0 &    0 &          3 &              67 &          178 &     69 &    179 \\
     aa11-er &                103 &             280 &                 2 &              0 &    1 &          8 &             100 &          273 &    103 &    280 \\
     aa13-er &                131 &             343 &                 6 &              0 &    2 &          6 &             123 &          324 &    131 &    343 \\
     aa14-er &                127 &             490 &                 1 &              0 &    0 &          0 &             126 &          489 &    127 &    490 \\
     aa15-er &                 67 &             171 &                 4 &              0 &    1 &          3 &              62 &          161 &     67 &    171 \\
     aa16-er &                 14 &              16 &                12 &              0 &    2 &          0 &               0 &            0 &     14 &     16 \\
     aa17-er &                153 &             582 &                 0 &              0 &    0 &          3 &             153 &          582 &    153 &    582 \\
     aa18-er &                 90 &             358 &                 0 &              0 &    0 &          0 &              90 &          358 &     90 &    358 \\
     aa19-er &                192 &             604 &                 1 &              0 &    0 &          4 &             191 &          603 &    192 &    604 \\
     aa20-er &                225 &             762 &                 0 &              0 &    0 &          5 &             225 &          762 &    225 &    762 \\
     aa21-er &                 31 &              80 &                 0 &              0 &    0 &          4 &              31 &           80 &     31 &     80 \\
     aa22-er &                167 &             598 &                 2 &              0 &    0 &          2 &             165 &          596 &    167 &    598 \\
     aa23-er &                143 &             466 &                 1 &              0 &    0 &          1 &             142 &          465 &    143 &    466 \\
     aa24-er &                261 &            1097 &                 1 &              0 &    0 &          1 &             260 &         1096 &    261 &   1097 \\
     aa25-er &                 15 &              16 &                 6 &              0 &    0 &          4 &               9 &           12 &     15 &     16 \\
     aa26-er &                 95 &             257 &                 3 &              0 &    0 &          6 &              92 &          254 &     95 &    257 \\
     aa27-er &                120 &             304 &                 3 &              0 &    0 &          7 &             117 &          301 &    120 &    304 \\
     aa28-er &                167 &             786 &                 1 &              0 &    0 &          0 &             166 &          785 &    167 &    786 \\
     aa29-er &                277 &            1034 &                 2 &              0 &    0 &          4 &             275 &         1033 &    277 &   1034 \\
     aa30-er &                 39 &              70 &                 5 &              0 &    0 &          5 &              34 &           65 &     39 &     70 \\
     aa31-er &                 30 &              53 &                 4 &              0 &    0 &          2 &              26 &           49 &     30 &     53 \\
     aa32-er &                151 &             699 &                 0 &              0 &    0 &          0 &             151 &          699 &    151 &    699 \\
     aa33-er &                194 &             460 &                 8 &              0 &    0 &         18 &             186 &          452 &    194 &    460 \\
     aa34-er &                134 &             413 &                 1 &              0 &    0 &          2 &             133 &          412 &    134 &    413 \\
     aa35-er &                 82 &             251 &                 3 &              0 &    2 &          4 &              77 &          235 &     82 &    251 \\
     aa36-er &                112 &             289 &                 3 &              0 &    0 &          4 &             109 &          287 &    112 &    289 \\
     aa37-er &                 73 &             150 &                 6 &              0 &    0 &         10 &              67 &          148 &     73 &    150 \\
     aa38-er &                171 &             787 &                 1 &              0 &    0 &          0 &             170 &          786 &    171 &    787 \\
     aa39-er &                145 &             651 &                 0 &              0 &    0 &          1 &             145 &          651 &    145 &    651 \\
     aa40-er &                140 &             569 &                 0 &              0 &    0 &          1 &             140 &          569 &    140 &    569 \\
     aa41-er &                300 &            1620 &                 0 &              0 &    0 &          0 &             300 &         1620 &    300 &   1620 \\
     aa42-er &                237 &            1068 &                 0 &              0 &    0 &          0 &             237 &         1068 &    237 &   1068 \\
     aa43-er &                 64 &             296 &                 0 &              0 &    0 &          0 &              64 &          296 &     64 &    296 \\
     aa44-er &                 60 &             151 &                 2 &              0 &    0 &          3 &              58 &          149 &     60 &    151 \\
     aa45-er &                 83 &             374 &                 0 &              0 &    0 &          0 &              83 &          374 &     83 &    374 \\
     aa46-er &                163 &             477 &                 4 &              0 &    0 &          6 &             159 &          473 &    163 &    477 \\
     aa47-er &                 65 &             215 &                 1 &              0 &    0 &          0 &              64 &          214 &     65 &    215 \\
     aa48-er &                 90 &             314 &                 0 &              0 &    0 &          1 &              90 &          314 &     90 &    314 \\
     aa49-er &                 27 &              59 &                 4 &              0 &    0 &          1 &              23 &           54 &     27 &     59 \\
     aa50-er &                113 &             437 &                 2 &              0 &    0 &          0 &             111 &          435 &    113 &    437 \\
     aa51-er &                 79 &             264 &                 1 &              0 &    0 &          5 &              78 &          263 &     79 &    264 \\
     aa52-er &                 66 &             215 &                 0 &              0 &    0 &          2 &              66 &          215 &     66 &    215 \\
     aa53-er &                 89 &             203 &                 5 &              0 &    0 &          8 &              84 &          198 &     89 &    203 \\
     aa54-er &                 90 &             205 &                 4 &              0 &    3 &          9 &              83 &          177 &     90 &    205 \\
  b-100_1-er &                100 &             444 &                 0 &              0 &    0 &          1 &             100 &          444 &    100 &    444 \\
 b-100_10-er &                100 &             461 &                 0 &              0 &    0 &          1 &             100 &          461 &    100 &    461 \\
  b-100_2-er &                100 &             459 &                 0 &              0 &    0 &          1 &             100 &          459 &    100 &    459 \\
  b-100_3-er &                100 &             467 &                 0 &              0 &    0 &          0 &             100 &          467 &    100 &    467 \\
  b-100_4-er &                100 &             451 &                 0 &              0 &    0 &          1 &             100 &          451 &    100 &    451 \\
  b-100_5-er &                100 &             433 &                 0 &              0 &    0 &          1 &             100 &          433 &    100 &    433 \\
  b-100_6-er &                100 &             499 &                 0 &              0 &    0 &          0 &             100 &          499 &    100 &    499 \\
  b-100_7-er &                100 &             445 &                 0 &              0 &    0 &          1 &             100 &          445 &    100 &    445 \\
  b-100_8-er &                100 &             470 &                 0 &              0 &    0 &          0 &             100 &          470 &    100 &    470 \\
  b-100_9-er &                100 &             486 &                 0 &              0 &    0 &          0 &             100 &          486 &    100 &    486 \\
   b-50_1-er &                 50 &             101 &                 7 &              0 &    1 &          6 &              42 &           87 &     50 &    101 \\
  b-50_10-er &                 50 &             101 &                 7 &              0 &    1 &          6 &              42 &           87 &     50 &    101 \\
   b-50_2-er &                 50 &             115 &                 2 &              0 &    1 &          5 &              47 &          107 &     50 &    115 \\
   b-50_3-er &                 50 &             127 &                 0 &              0 &    0 &          2 &              50 &          127 &     50 &    127 \\
   b-50_4-er &                 50 &             102 &                 5 &              0 &    1 &          7 &              44 &           91 &     50 &    102 \\
   b-50_5-er &                 50 &             126 &                 0 &              0 &    0 &          2 &              50 &          126 &     50 &    126 \\
   b-50_6-er &                 50 &              94 &                 9 &              0 &    1 &          7 &              40 &           78 &     50 &     94 \\
   b-50_7-er &                 50 &             122 &                 1 &              0 &    1 &          3 &              48 &          115 &     50 &    122 \\
   b-50_8-er &                 50 &             135 &                 0 &              0 &    0 &          1 &              50 &          135 &     50 &    135 \\
   b-50_9-er &                 50 &             120 &                 1 &              0 &    1 &          4 &              48 &          113 &     50 &    120 \\
    gka_1-er &                 50 &              98 &                 8 &              0 &    0 &          7 &              42 &           88 &     50 &     98 \\
   gka_10-er &                 30 &             426 &                 0 &              0 &   22 &          0 &               8 &           24 &     30 &    426 \\
   gka_11-er &                 40 &             768 &                 0 &              0 &   28 &          0 &              12 &           60 &     40 &    768 \\
   gka_12-er &                 50 &            1205 &                 0 &              0 &   32 &          0 &              18 &          144 &     50 &   1205 \\
   gka_13-er &                 60 &            1748 &                 0 &              0 &   44 &          0 &              16 &          112 &     60 &   1748 \\
   gka_14-er &                 70 &            2383 &                 4 &              0 &   66 &          0 &               0 &            0 &     70 &   2383 \\
   gka_15-er &                 80 &            3114 &                 4 &              0 &   76 &          0 &               0 &            0 &     80 &   3114 \\
   gka_16-er &                 90 &            3956 &                 0 &              0 &   83 &          1 &               7 &           16 &     90 &   3956 \\
   gka_17-er &                100 &            4895 &                 0 &              0 &   72 &          0 &              28 &          364 &    100 &   4895 \\
   gka_18-er &                125 &            7661 &                 4 &              0 &  121 &          0 &               0 &            0 &    125 &   7661 \\
   gka_19-er &                 40 &             624 &                 0 &              0 &    0 &          0 &              40 &          624 &     40 &    624 \\
    gka_2-er &                 60 &             151 &                 2 &              0 &    0 &          3 &              58 &          149 &     60 &    151 \\
   gka_20-er &                 50 &             751 &                 0 &              0 &    0 &          0 &              50 &          751 &     50 &    751 \\
   gka_21-er &                 60 &             676 &                 0 &              0 &    0 &          0 &              60 &          676 &     60 &    676 \\
   gka_22-er &                 70 &             687 &                 0 &              0 &    0 &          0 &              70 &          687 &     70 &    687 \\
   gka_23-er &                 80 &             621 &                 0 &              0 &    0 &          0 &              80 &          621 &     80 &    621 \\
   gka_24-er &                 90 &             380 &                 0 &              0 &    0 &          0 &              90 &          380 &     90 &    380 \\
   gka_25-er &                100 &             474 &                 0 &              0 &    0 &          0 &             100 &          474 &    100 &    474 \\
   gka_26-er &                100 &             472 &                 0 &              0 &    0 &          0 &             100 &          472 &    100 &    472 \\
   gka_27-er &                100 &            1001 &                 0 &              0 &    0 &          0 &             100 &         1001 &    100 &   1001 \\
   gka_28-er &                100 &            1415 &                 0 &              0 &    0 &          0 &             100 &         1415 &    100 &   1415 \\
   gka_29-er &                100 &            1992 &                 0 &              0 &    0 &          0 &             100 &         1992 &    100 &   1992 \\
    gka_3-er &                 70 &             206 &                 2 &              0 &    0 &          2 &              68 &          205 &     70 &    206 \\
   gka_30-er &                100 &            2382 &                 0 &              0 &    0 &          0 &             100 &         2382 &    100 &   2382 \\
   gka_31-er &                100 &            2942 &                 0 &              0 &    0 &          0 &             100 &         2942 &    100 &   2942 \\
   gka_32-er &                100 &            3449 &                 0 &              0 &    0 &          0 &             100 &         3449 &    100 &   3449 \\
   gka_33-er &                100 &            3931 &                 0 &              0 &    0 &          0 &             100 &         3931 &    100 &   3931 \\
   gka_34-er &                100 &            4388 &                 0 &              0 &    0 &          0 &             100 &         4388 &    100 &   4388 \\
   gka_35-er &                100 &            4889 &                 0 &              0 &   93 &          0 &               7 &           15 &    100 &   4889 \\
    gka_4-er &                 80 &             293 &                 0 &              0 &    0 &          3 &              80 &          293 &     80 &    293 \\
    gka_5-er &                 50 &             219 &                 0 &              0 &    0 &          0 &              50 &          219 &     50 &    219 \\
    gka_6-er &                 30 &             177 &                 0 &              0 &    0 &          0 &              30 &          177 &     30 &    177 \\
    gka_7-er &                 30 &             213 &                 0 &              0 &    0 &          0 &              30 &          213 &     30 &    213 \\
    gka_8-er &                100 &             275 &                 3 &              0 &    0 &          3 &              97 &          272 &    100 &    275 \\
    gka_9-er &                 20 &             186 &                 4 &              0 &   16 &          0 &               0 &            0 &     20 &    186 \\
      j10-er &                 57 &             106 &                 7 &              0 &    0 &         10 &              50 &          100 &     57 &    106 \\
      j11-er &                 51 &             205 &                 0 &              0 &    0 &          0 &              51 &          205 &     51 &    205 \\
      j13-er &                 78 &             192 &                 0 &              0 &    0 &          7 &              78 &          192 &     78 &    192 \\
      j14-er &                 72 &              87 &                48 &              0 &    3 &          8 &              22 &           34 &     72 &     87 \\
      j15-er &                 45 &              45 &                44 &              1 &    3 &          0 &               0 &            0 &     45 &     45 \\
      j16-er &                 14 &              14 &                12 &              2 &    2 &          0 &               0 &            0 &     14 &     14 \\
      j17-er &                 81 &             312 &                 0 &              0 &    0 &          1 &              81 &          312 &     81 &    312 \\
      j18-er &                 73 &             280 &                 1 &              0 &    0 &          3 &              72 &          279 &     73 &    280 \\
      j19-er &                101 &             161 &                40 &              0 &    4 &          9 &              58 &          107 &    101 &    161 \\
      j20-er &                241 &             620 &                 9 &              0 &    0 &         19 &             232 &          612 &    241 &    620 \\
      j21-er &                 33 &              92 &                 0 &              0 &    0 &          2 &              33 &           92 &     33 &     92 \\
      j22-er &                 76 &             387 &                 0 &              0 &    0 &          0 &              76 &          387 &     76 &    387 \\
      j23-er &                 76 &             364 &                 0 &              0 &    0 &          0 &              76 &          364 &     76 &    364 \\
      j24-er &                150 &             357 &                 6 &              0 &    0 &          9 &             144 &          352 &    150 &    357 \\
      j25-er &                 14 &              14 &                12 &              2 &    2 &          0 &               0 &            0 &     14 &     14 \\
      j26-er &                 65 &             140 &                 4 &              0 &    0 &          8 &              62 &          137 &     65 &    140 \\
      j28-er &                 96 &             553 &                 0 &              0 &    0 &          1 &              96 &          553 &     96 &    553 \\
     aa10-cl &                 69 &             172 &                31 &              0 &    5 &          6 &              34 &           72 &     69 &    172 \\
     aa11-cl &                103 &             299 &                42 &              0 &    0 &          9 &              61 &          275 &    103 &    299 \\
     aa13-cl &                131 &             370 &                48 &              0 &    3 &         28 &              80 &          266 &    131 &    370 \\
     aa14-cl &                127 &             521 &                51 &              0 &    8 &         12 &              68 &          322 &    127 &    521 \\
     aa15-cl &                 67 &             167 &                35 &              0 &    6 &          4 &              26 &           68 &     67 &    167 \\
     aa16-cl &                 14 &              15 &                12 &              0 &    2 &          0 &               0 &            0 &     14 &     15 \\
     aa17-cl &                153 &             658 &                60 &              0 &    8 &         15 &              85 &          383 &    153 &    658 \\
     aa18-cl &                 90 &             350 &                31 &              0 &    1 &          5 &              58 &          313 &     90 &    350 \\
     aa19-cl &                192 &             670 &                85 &              0 &    9 &         23 &              98 &          381 &    192 &    670 \\
     aa20-cl &                225 &             777 &               100 &              0 &    9 &         28 &             116 &          440 &    225 &    777 \\
     aa21-cl &                 31 &              91 &                13 &              0 &    6 &          2 &              12 &           25 &     31 &     91 \\
     aa22-cl &                167 &             665 &                71 &              0 &    8 &         13 &              88 &          416 &    167 &    665 \\
     aa23-cl &                143 &             506 &                68 &              0 &   11 &         15 &              64 &          210 &    143 &    506 \\
     aa24-cl &                261 &            1110 &               128 &              0 &   16 &         29 &             117 &          494 &    261 &   1110 \\
     aa25-cl &                 15 &              15 &                13 &              0 &    2 &          0 &               0 &            0 &     15 &     15 \\
     aa26-cl &                 95 &             302 &                28 &              0 &    3 &         13 &              64 &          237 &     95 &    302 \\
     aa27-cl &                120 &             343 &                49 &              0 &    5 &         10 &              66 &          217 &    120 &    343 \\
     aa28-cl &                167 &             849 &                72 &              0 &   13 &         17 &              82 &          377 &    167 &    849 \\
     aa29-cl &                277 &            1082 &               145 &              0 &   17 &         32 &             115 &          452 &    277 &   1082 \\
     aa30-cl &                 39 &              66 &                21 &              0 &    2 &          3 &              16 &           30 &     39 &     66 \\
     aa31-cl &                 30 &              51 &                25 &              0 &    5 &          0 &               0 &            0 &     30 &     51 \\
     aa32-cl &                151 &             747 &                56 &              0 &    5 &         12 &              90 &          548 &    151 &    747 \\
     aa33-cl &                194 &             478 &               112 &              0 &    9 &         15 &              73 &          202 &    194 &    478 \\
     aa34-cl &                134 &             444 &                71 &              0 &   15 &         12 &              48 &          142 &    134 &    444 \\
     aa35-cl &                 82 &             275 &                27 &              0 &    1 &          5 &              54 &          239 &     82 &    275 \\
     aa36-cl &                112 &             334 &                48 &              0 &    4 &          9 &              60 &          233 &    112 &    334 \\
     aa37-cl &                 73 &             166 &                36 &              0 &    5 &         10 &              32 &           69 &     73 &    166 \\
     aa38-cl &                171 &             876 &                78 &              0 &   21 &         11 &              72 &          294 &    171 &    876 \\
     aa39-cl &                145 &             683 &                57 &              0 &   13 &         14 &              75 &          321 &    145 &    683 \\
     aa40-cl &                140 &             611 &                55 &              0 &    6 &         13 &              79 &          446 &    140 &    611 \\
     aa41-cl &                300 &            1626 &               148 &              0 &   19 &         33 &             134 &          768 &    300 &   1626 \\
     aa42-cl &                237 &            1144 &               107 &              0 &   17 &         23 &             113 &          504 &    237 &   1144 \\
     aa43-cl &                 64 &             287 &                15 &              0 &    3 &          5 &              46 &          218 &     64 &    287 \\
     aa44-cl &                 60 &             162 &                16 &              0 &    2 &          8 &              42 &          124 &     60 &    162 \\
     aa45-cl &                 83 &             366 &                21 &              0 &    1 &          5 &              61 &          335 &     83 &    366 \\
     aa46-cl &                163 &             528 &                61 &              0 &    3 &         19 &              99 &          445 &    163 &    528 \\
     aa47-cl &                 65 &             223 &                25 &              0 &    4 &          3 &              36 &          148 &     65 &    223 \\
     aa48-cl &                 90 &             346 &                30 &              0 &    3 &         12 &              57 &          253 &     90 &    346 \\
     aa49-cl &                 27 &              58 &                22 &              0 &    5 &          0 &               0 &            0 &     27 &     58 \\
     aa50-cl &                113 &             448 &                39 &              0 &    6 &          8 &              68 &          289 &    113 &    448 \\
     aa51-cl &                 79 &             272 &                18 &              0 &    2 &          9 &              59 &          218 &     79 &    272 \\
     aa52-cl &                 66 &             229 &                19 &              0 &    2 &          4 &              45 &          184 &     66 &    229 \\
     aa53-cl &                 89 &             223 &                25 &              0 &    1 &         13 &              63 &          190 &     89 &    223 \\
     aa54-cl &                 90 &             239 &                28 &              0 &    2 &          9 &              60 &          192 &     90 &    239 \\
  b-100_1-cl &                100 &             483 &                 1 &              0 &    0 &          2 &              99 &          482 &    100 &    483 \\
 b-100_10-cl &                100 &             481 &                 2 &              0 &    1 &          3 &              97 &          465 &    100 &    481 \\
  b-100_2-cl &                100 &             508 &                 1 &              0 &    1 &          0 &              98 &          500 &    100 &    508 \\
  b-100_3-cl &                100 &             498 &                 0 &              0 &    0 &          0 &             100 &          498 &    100 &    498 \\
  b-100_4-cl &                100 &             506 &                 0 &              0 &    0 &          2 &             100 &          506 &    100 &    506 \\
  b-100_5-cl &                100 &             475 &                 2 &              0 &    1 &          1 &              97 &          458 &    100 &    475 \\
  b-100_6-cl &                100 &             512 &                 1 &              0 &    1 &          2 &              98 &          495 &    100 &    512 \\
  b-100_7-cl &                100 &             470 &                 4 &              0 &    1 &          0 &              95 &          459 &    100 &    470 \\
  b-100_8-cl &                100 &             504 &                 0 &              0 &    0 &          0 &             100 &          504 &    100 &    504 \\
  b-100_9-cl &                100 &             510 &                 0 &              0 &    0 &          1 &             100 &          510 &    100 &    510 \\
   b-50_1-cl &                 50 &             106 &                 4 &              0 &    0 &         11 &              46 &          103 &     50 &    106 \\
  b-50_10-cl &                 50 &              98 &                13 &              0 &    1 &          8 &              36 &           77 &     50 &     98 \\
   b-50_2-cl &                 50 &             123 &                 5 &              0 &    0 &          5 &              45 &          120 &     50 &    123 \\
   b-50_3-cl &                 50 &             125 &                 5 &              0 &    0 &          3 &              45 &          120 &     50 &    125 \\
   b-50_4-cl &                 50 &             114 &                10 &              0 &    1 &          3 &              39 &          102 &     50 &    114 \\
   b-50_5-cl &                 50 &             127 &                 4 &              0 &    1 &          6 &              45 &          117 &     50 &    127 \\
   b-50_6-cl &                 50 &             101 &                12 &              0 &    1 &          5 &              37 &           86 &     50 &    101 \\
   b-50_7-cl &                 50 &             117 &                 6 &              0 &    2 &          7 &              42 &          101 &     50 &    117 \\
   b-50_8-cl &                 50 &             137 &                 0 &              0 &    0 &          2 &              50 &          137 &     50 &    137 \\
   b-50_9-cl &                 50 &             125 &                 8 &              0 &    0 &          4 &              42 &          117 &     50 &    125 \\
    gka_1-cl &                 50 &             103 &                10 &              0 &    1 &          5 &              39 &           84 &     50 &    103 \\
   gka_10-cl &                 30 &             416 &                 4 &              0 &   26 &          0 &               0 &            0 &     30 &    416 \\
   gka_11-cl &                 40 &             757 &                 0 &              0 &   32 &          0 &               8 &           24 &     40 &    757 \\
   gka_12-cl &                 50 &            1191 &                 5 &              0 &   45 &          0 &               0 &            0 &     50 &   1191 \\
   gka_13-cl &                 60 &            1719 &                 0 &              0 &   41 &          0 &              19 &          151 &     60 &   1719 \\
   gka_14-cl &                 70 &            2352 &                 0 &              0 &   58 &          0 &              12 &           49 &     70 &   2352 \\
   gka_15-cl &                 80 &            3075 &                 0 &              0 &   28 &          0 &              52 &         1256 &     80 &   3075 \\
   gka_16-cl &                 90 &            3920 &                 0 &              0 &   45 &          0 &              45 &          931 &     90 &   3920 \\
   gka_17-cl &                100 &            4855 &                 5 &              0 &   95 &          0 &               0 &            0 &    100 &   4855 \\
   gka_18-cl &                125 &            7602 &                 0 &              0 &   59 &          0 &              66 &         2041 &    125 &   7602 \\
   gka_19-cl &                 40 &             609 &                 0 &              0 &    3 &          0 &              37 &          505 &     40 &    609 \\
    gka_2-cl &                 60 &             154 &                 9 &              0 &    0 &          3 &              51 &          148 &     60 &    154 \\
   gka_20-cl &                 50 &             735 &                 0 &              0 &    0 &          0 &              50 &          735 &     50 &    735 \\
   gka_21-cl &                 60 &             675 &                 0 &              0 &    0 &          0 &              60 &          675 &     60 &    675 \\
   gka_22-cl &                 70 &             735 &                 0 &              0 &    0 &          0 &              70 &          735 &     70 &    735 \\
   gka_23-cl &                 80 &             650 &                 0 &              0 &    0 &          0 &              80 &          650 &     80 &    650 \\
   gka_24-cl &                 90 &             434 &                 0 &              0 &    0 &          2 &              90 &          434 &     90 &    434 \\
   gka_25-cl &                100 &             504 &                 1 &              0 &    0 &          2 &              99 &          503 &    100 &    504 \\
   gka_26-cl &                100 &             507 &                 1 &              0 &    0 &          1 &              99 &          506 &    100 &    507 \\
   gka_27-cl &                100 &            1021 &                 0 &              0 &    0 &          0 &             100 &         1021 &    100 &   1021 \\
   gka_28-cl &                100 &            1427 &                 0 &              0 &    0 &          0 &             100 &         1427 &    100 &   1427 \\
   gka_29-cl &                100 &            2007 &                 0 &              0 &    0 &          0 &             100 &         2007 &    100 &   2007 \\
    gka_3-cl &                 70 &             215 &                 2 &              0 &    0 &          2 &              68 &          213 &     70 &    215 \\
   gka_30-cl &                100 &            2410 &                 0 &              0 &    0 &          0 &             100 &         2410 &    100 &   2410 \\
   gka_31-cl &                100 &            2972 &                 0 &              0 &    0 &          0 &             100 &         2972 &    100 &   2972 \\
   gka_32-cl &                100 &            3382 &                 0 &              0 &    0 &          0 &             100 &         3382 &    100 &   3382 \\
   gka_33-cl &                100 &            3849 &                 0 &              0 &    0 &          0 &             100 &         3849 &    100 &   3849 \\
   gka_34-cl &                100 &            4273 &                 0 &              0 &    1 &          0 &              99 &         4177 &    100 &   4273 \\
   gka_35-cl &                100 &            4861 &                 4 &              0 &   96 &          0 &               0 &            0 &    100 &   4861 \\
    gka_4-cl &                 80 &             299 &                 2 &              0 &    0 &          5 &              78 &          297 &     80 &    299 \\
    gka_5-cl &                 50 &             226 &                 0 &              0 &    0 &          1 &              50 &          226 &     50 &    226 \\
    gka_6-cl &                 30 &             166 &                 0 &              0 &    0 &          0 &              30 &          166 &     30 &    166 \\
    gka_7-cl &                 30 &             209 &                 0 &              0 &    0 &          0 &              30 &          209 &     30 &    209 \\
    gka_8-cl &                100 &             310 &                 3 &              0 &    0 &          5 &              97 &          309 &    100 &    310 \\
    gka_9-cl &                 20 &             178 &                 4 &              0 &   16 &          0 &               0 &            0 &     20 &    178 \\
      j10-cl &                 57 &             120 &                28 &              0 &    4 &          7 &              25 &           51 &     57 &    120 \\
      j11-cl &                 51 &             206 &                16 &              0 &    1 &          2 &              34 &          176 &     51 &    206 \\
      j13-cl &                 78 &             189 &                37 &              0 &    3 &          7 &              38 &          117 &     78 &    189 \\
      j14-cl &                 72 &              95 &                47 &              0 &    3 &          7 &              22 &           41 &     72 &     95 \\
      j15-cl &                 45 &              46 &                43 &              0 &    2 &          0 &               0 &            0 &     45 &     46 \\
      j16-cl &                 14 &               9 &                13 &              0 &    1 &          0 &               0 &            0 &     14 &      9 \\
      j17-cl &                 81 &             308 &                40 &              0 &    9 &          3 &              32 &          110 &     81 &    308 \\
      j18-cl &                 73 &             279 &                19 &              0 &    3 &          7 &              51 &          208 &     73 &    279 \\
      j19-cl &                101 &             175 &                68 &              0 &    6 &          9 &              27 &           55 &    101 &    175 \\
      j20-cl &                241 &             670 &                94 &              0 &    5 &         37 &             144 &          476 &    241 &    670 \\
      j21-cl &                 33 &             104 &                15 &              0 &    5 &          0 &              13 &           38 &     33 &    104 \\
      j22-cl &                 76 &             409 &                11 &              0 &    1 &          2 &              64 &          380 &     76 &    409 \\
      j23-cl &                 76 &             384 &                19 &              0 &    0 &          5 &              57 &          373 &     76 &    384 \\
      j24-cl &                150 &             365 &                67 &              0 &    3 &         17 &              80 &          268 &    150 &    365 \\
      j25-cl &                 14 &              15 &                13 &              0 &    1 &          0 &               0 &            0 &     14 &     15 \\
      j26-cl &                 65 &             157 &                27 &              0 &    2 &          7 &              36 &          112 &     65 &    157 \\
      j28-cl &                 96 &             589 &                32 &              0 &    4 &          4 &              60 &          466 &     96 &    589 \\
     aa10-ba &                 69 &             198 &                 0 &              0 &    0 &          0 &              69 &          198 &     69 &    198 \\
     aa10-to &                 69 &             114 &                 9 &              0 &    0 &         13 &              60 &          108 &     69 &    114 \\
     aa11-ba &                103 &             300 &                 0 &              0 &    0 &          0 &             103 &          300 &    103 &    300 \\
     aa11-to &                103 &             169 &                24 &              0 &    0 &         19 &              79 &          149 &    103 &    169 \\
     aa13-ba &                131 &             384 &                 0 &              0 &    0 &          0 &             131 &          384 &    131 &    384 \\
     aa13-to &                131 &             196 &                46 &              0 &    1 &         27 &              86 &          148 &    131 &    196 \\
     aa14-ba &                127 &             610 &                 0 &              0 &    0 &          0 &             127 &          610 &    127 &    610 \\
     aa14-to &                127 &             304 &                11 &              0 &    0 &         10 &             116 &          294 &    127 &    304 \\
     aa15-ba &                 67 &             192 &                 0 &              0 &    0 &          0 &              67 &          192 &     67 &    192 \\
     aa15-to &                 67 &             105 &                19 &              0 &    0 &         11 &              49 &           90 &     67 &    105 \\
     aa16-ba &                 14 &              24 &                12 &              0 &    2 &          0 &               0 &            0 &     14 &     24 \\
     aa16-to &                 14 &               9 &                14 &              0 &    0 &          0 &               0 &            0 &     14 &      9 \\
     aa17-ba &                153 &             740 &                 0 &              0 &    0 &          0 &             153 &          740 &    153 &    740 \\
     aa17-to &                153 &             363 &                16 &              0 &    1 &         19 &             136 &          340 &    153 &    363 \\
     aa18-ba &                 90 &             425 &                 0 &              0 &    0 &          0 &              90 &          425 &     90 &    425 \\
     aa18-to &                 90 &             233 &                 7 &              0 &    0 &          6 &              83 &          228 &     90 &    233 \\
     aa19-ba &                192 &             752 &                 0 &              0 &    0 &          0 &             192 &          752 &    192 &    752 \\
     aa19-to &                192 &             366 &                38 &              0 &    1 &         26 &             153 &          322 &    192 &    366 \\
     aa20-ba &                225 &             884 &                 0 &              0 &    0 &          0 &             225 &          884 &    225 &    884 \\
     aa20-to &                225 &             437 &                33 &              0 &    0 &         31 &             193 &          408 &    225 &    437 \\
     aa21-ba &                 31 &              84 &                 0 &              0 &    0 &          0 &              31 &           84 &     31 &     84 \\
     aa21-to &                 31 &              62 &                 4 &              0 &    0 &          6 &              27 &           58 &     31 &     62 \\
     aa22-ba &                167 &             652 &                 0 &              0 &    0 &          0 &             167 &          652 &    167 &    652 \\
     aa22-to &                167 &             365 &                13 &              0 &    0 &         19 &             154 &          356 &    167 &    365 \\
     aa23-ba &                143 &             556 &                 0 &              0 &    0 &          0 &             143 &          556 &    143 &    556 \\
     aa23-to &                143 &             286 &                18 &              0 &    0 &         25 &             125 &          269 &    143 &    286 \\
     aa24-ba &                261 &            1280 &                 0 &              0 &    0 &          0 &             261 &         1280 &    261 &   1280 \\
     aa24-to &                261 &             618 &                17 &              0 &    0 &         18 &             244 &          605 &    261 &    618 \\
     aa25-ba &                 15 &              14 &                15 &              0 &    0 &          0 &               0 &            0 &     15 &     14 \\
     aa25-to &                 15 &               7 &                15 &              0 &    0 &          0 &               0 &            0 &     15 &      7 \\
     aa26-ba &                 95 &             276 &                 0 &              0 &    0 &          0 &              95 &          276 &     95 &    276 \\
     aa26-to &                 95 &             157 &                24 &              0 &    1 &         19 &              70 &          132 &     95 &    157 \\
     aa27-ba &                120 &             351 &                 0 &              0 &    0 &          0 &             120 &          351 &    120 &    351 \\
     aa27-to &                120 &             172 &                57 &              0 &    2 &         17 &              62 &          108 &    120 &    172 \\
     aa28-ba &                167 &             966 &                 0 &              0 &    0 &          0 &             167 &          966 &    167 &    966 \\
     aa28-to &                167 &             521 &                 3 &              0 &    0 &          8 &             164 &          519 &    167 &    521 \\
     aa29-ba &                277 &            1092 &                 0 &              0 &    0 &          0 &             277 &         1092 &    277 &   1092 \\
     aa29-to &                277 &             583 &                27 &              0 &    0 &         33 &             250 &          559 &    277 &    583 \\
     aa30-ba &                 39 &              74 &                35 &              0 &    5 &          0 &               0 &            0 &     39 &     74 \\
     aa30-to &                 39 &              50 &                18 &              0 &    0 &          6 &              22 &           36 &     39 &     50 \\
     aa31-ba &                 30 &              56 &                26 &              0 &    5 &          0 &               0 &            0 &     30 &     56 \\
     aa31-to &                 30 &              30 &                30 &              0 &    1 &          0 &               0 &            0 &     30 &     30 \\
     aa32-ba &                151 &             730 &                 0 &              0 &    0 &          0 &             151 &          730 &    151 &    730 \\
     aa32-to &                151 &             466 &                 3 &              0 &    0 &          6 &             148 &          463 &    151 &    466 \\
     aa33-ba &                194 &             573 &                 0 &              0 &    0 &          0 &             194 &          573 &    194 &    573 \\
     aa33-to &                194 &             252 &                88 &              0 &    0 &         29 &             110 &          182 &    194 &    252 \\
     aa34-ba &                134 &             520 &                 0 &              0 &    0 &          0 &             134 &          520 &    134 &    520 \\
     aa34-to &                134 &             243 &                29 &              0 &    0 &         17 &             105 &          218 &    134 &    243 \\
     aa35-ba &                 82 &             312 &                 0 &              0 &    0 &          0 &              82 &          312 &     82 &    312 \\
     aa35-to &                 82 &             163 &                 9 &              0 &    0 &         10 &              73 &          154 &     82 &    163 \\
     aa36-ba &                112 &             327 &                 0 &              0 &    0 &          0 &             112 &          327 &    112 &    327 \\
     aa36-to &                112 &             163 &                35 &              0 &    0 &         19 &              77 &          136 &    112 &    163 \\
     aa37-ba &                 73 &             210 &                 7 &              0 &    4 &         12 &              62 &          133 &     73 &    210 \\
     aa37-to &                 73 &              93 &                38 &              0 &    2 &         11 &              34 &           56 &     73 &     93 \\
     aa38-ba &                171 &             990 &                 0 &              0 &    0 &          0 &             171 &          990 &    171 &    990 \\
     aa38-to &                171 &             498 &                 7 &              0 &    2 &          4 &             162 &          480 &    171 &    498 \\
     aa39-ba &                145 &             700 &                 0 &              0 &    0 &          0 &             145 &          700 &    145 &    700 \\
     aa39-to &                145 &             408 &                 6 &              0 &    0 &          9 &             139 &          401 &    145 &    408 \\
     aa40-ba &                140 &             675 &                 0 &              0 &    0 &          0 &             140 &          675 &    140 &    675 \\
     aa40-to &                140 &             357 &                 9 &              0 &    1 &         13 &             130 &          341 &    140 &    357 \\
     aa41-ba &                300 &            1764 &                 0 &              0 &    0 &          0 &             300 &         1764 &    300 &   1764 \\
     aa41-to &                300 &            1014 &                 0 &              0 &    0 &         10 &             300 &         1014 &    300 &   1014 \\
     aa42-ba &                237 &            1160 &                 0 &              0 &    0 &          0 &             237 &         1160 &    237 &   1160 \\
     aa42-to &                237 &             646 &                10 &              0 &    1 &         17 &             226 &          623 &    237 &    646 \\
     aa43-ba &                 64 &             295 &                 0 &              0 &    0 &          0 &              64 &          295 &     64 &    295 \\
     aa43-to &                 64 &             217 &                 0 &              0 &    0 &          0 &              64 &          217 &     64 &    217 \\
     aa44-ba &                 60 &             171 &                 0 &              0 &    0 &          0 &              60 &          171 &     60 &    171 \\
     aa44-to &                 60 &             104 &                10 &              0 &    0 &         15 &              50 &           96 &     60 &    104 \\
     aa45-ba &                 83 &             390 &                 0 &              0 &    0 &          0 &              83 &          390 &     83 &    390 \\
     aa45-to &                 83 &             263 &                 2 &              0 &    0 &          1 &              81 &          261 &     83 &    263 \\
     aa46-ba &                163 &             636 &                 0 &              0 &    0 &          0 &             163 &          636 &    163 &    636 \\
     aa46-to &                163 &             275 &                35 &              0 &    0 &         25 &             130 &          246 &    163 &    275 \\
     aa47-ba &                 65 &             244 &                 0 &              0 &    1 &          0 &              64 &          230 &     65 &    244 \\
     aa47-to &                 65 &             151 &                 8 &              0 &    1 &          7 &              56 &          135 &     65 &    151 \\
     aa48-ba &                 90 &             344 &                 0 &              0 &    0 &          0 &              90 &          344 &     90 &    344 \\
     aa48-to &                 90 &             207 &                 6 &              0 &    0 &          9 &              84 &          201 &     90 &    207 \\
     aa49-ba &                 27 &              72 &                 0 &              0 &    0 &          0 &              27 &           72 &     27 &     72 \\
     aa49-to &                 27 &              41 &                 5 &              0 &    0 &          3 &              22 &           38 &     27 &     41 \\
     aa50-ba &                113 &             540 &                 0 &              0 &    0 &          0 &             113 &          540 &    113 &    540 \\
     aa50-to &                113 &             287 &                 5 &              0 &    0 &          7 &             108 &          283 &    113 &    287 \\
     aa51-ba &                 79 &             300 &                 0 &              0 &    0 &          0 &              79 &          300 &     79 &    300 \\
     aa51-to &                 79 &             170 &                 8 &              0 &    0 &          8 &              71 &          163 &     79 &    170 \\
     aa52-ba &                 66 &             248 &                 0 &              0 &    1 &          0 &              65 &          234 &     66 &    248 \\
     aa52-to &                 66 &             153 &                 7 &              0 &    0 &          6 &              59 &          147 &     66 &    153 \\
     aa53-ba &                 89 &             258 &                 0 &              0 &    0 &          0 &              89 &          258 &     89 &    258 \\
     aa53-to &                 89 &             125 &                26 &              0 &    0 &         17 &              63 &          106 &     89 &    125 \\
     aa54-ba &                 90 &             261 &                 0 &              0 &    0 &          0 &              90 &          261 &     90 &    261 \\
     aa54-to &                 90 &             123 &                29 &              0 &    0 &         16 &              62 &          101 &     90 &    123 \\
  b-100_1-ba &                100 &             475 &                 0 &              0 &    0 &          0 &             100 &          475 &    100 &    475 \\
  b-100_1-to &                100 &             374 &                 0 &              0 &    0 &          3 &             100 &          374 &    100 &    374 \\
 b-100_10-ba &                100 &             475 &                 0 &              0 &    0 &          0 &             100 &          475 &    100 &    475 \\
 b-100_10-to &                100 &             389 &                 0 &              0 &    0 &          1 &             100 &          389 &    100 &    389 \\
  b-100_2-ba &                100 &             475 &                 0 &              0 &    0 &          0 &             100 &          475 &    100 &    475 \\
  b-100_2-to &                100 &             395 &                 1 &              0 &    0 &          1 &              99 &          394 &    100 &    395 \\
  b-100_3-ba &                100 &             475 &                 0 &              0 &    0 &          0 &             100 &          475 &    100 &    475 \\
  b-100_3-to &                100 &             401 &                 1 &              0 &    0 &          0 &              99 &          400 &    100 &    401 \\
  b-100_4-ba &                100 &             475 &                 0 &              0 &    0 &          0 &             100 &          475 &    100 &    475 \\
  b-100_4-to &                100 &             380 &                 0 &              0 &    0 &          3 &             100 &          380 &    100 &    380 \\
  b-100_5-ba &                100 &             475 &                 0 &              0 &    0 &          0 &             100 &          475 &    100 &    475 \\
  b-100_5-to &                100 &             370 &                 1 &              0 &    0 &          2 &              99 &          369 &    100 &    370 \\
  b-100_6-ba &                100 &             564 &                 0 &              0 &    0 &          0 &             100 &          564 &    100 &    564 \\
  b-100_6-to &                100 &             418 &                 0 &              0 &    0 &          0 &             100 &          418 &    100 &    418 \\
  b-100_7-ba &                100 &             475 &                 0 &              0 &    0 &          0 &             100 &          475 &    100 &    475 \\
  b-100_7-to &                100 &             382 &                 1 &              0 &    0 &          2 &              99 &          381 &    100 &    382 \\
  b-100_8-ba &                100 &             475 &                 0 &              0 &    0 &          0 &             100 &          475 &    100 &    475 \\
  b-100_8-to &                100 &             395 &                 0 &              0 &    0 &          0 &             100 &          395 &    100 &    395 \\
  b-100_9-ba &                100 &             564 &                 0 &              0 &    0 &          0 &             100 &          564 &    100 &    564 \\
  b-100_9-to &                100 &             409 &                 0 &              0 &    0 &          0 &             100 &          409 &    100 &    409 \\
   b-50_1-ba &                 50 &             141 &                 0 &              0 &    0 &          0 &              50 &          141 &     50 &    141 \\
   b-50_1-to &                 50 &              68 &                22 &              0 &    1 &          7 &              27 &           49 &     50 &     68 \\
  b-50_10-ba &                 50 &             141 &                 0 &              0 &    0 &          0 &              50 &          141 &     50 &    141 \\
  b-50_10-to &                 50 &              68 &                22 &              0 &    1 &          7 &              27 &           49 &     50 &     68 \\
   b-50_2-ba &                 50 &             141 &                 0 &              0 &    0 &          0 &              50 &          141 &     50 &    141 \\
   b-50_2-to &                 50 &              77 &                15 &              0 &    0 &         10 &              36 &           66 &     50 &     77 \\
   b-50_3-ba &                 50 &             141 &                 0 &              0 &    0 &          0 &              50 &          141 &     50 &    141 \\
   b-50_3-to &                 50 &              99 &                 5 &              0 &    0 &          5 &              45 &           96 &     50 &     99 \\
   b-50_4-ba &                 50 &             141 &                 0 &              0 &    0 &          0 &              50 &          141 &     50 &    141 \\
   b-50_4-to &                 50 &              69 &                22 &              0 &    1 &          7 &              27 &           49 &     50 &     69 \\
   b-50_5-ba &                 50 &             141 &                 0 &              0 &    0 &          0 &              50 &          141 &     50 &    141 \\
   b-50_5-to &                 50 &             106 &                 6 &              0 &    0 &          4 &              44 &          100 &     50 &    106 \\
   b-50_6-ba &                 50 &             141 &                 0 &              0 &    0 &          0 &              50 &          141 &     50 &    141 \\
   b-50_6-to &                 50 &              61 &                27 &              0 &    0 &          7 &              23 &           37 &     50 &     61 \\
   b-50_7-ba &                 50 &             141 &                 0 &              0 &    0 &          0 &              50 &          141 &     50 &    141 \\
   b-50_7-to &                 50 &              92 &                 3 &              0 &    0 &         12 &              47 &           89 &     50 &     92 \\
   b-50_8-ba &                 50 &             141 &                 0 &              0 &    0 &          0 &              50 &          141 &     50 &    141 \\
   b-50_8-to &                 50 &             106 &                 5 &              0 &    0 &          3 &              45 &          103 &     50 &    106 \\
   b-50_9-ba &                 50 &             141 &                 0 &              0 &    0 &          0 &              50 &          141 &     50 &    141 \\
   b-50_9-to &                 50 &              89 &                 8 &              0 &    1 &          7 &              41 &           75 &     50 &     89 \\
    gka_1-ba &                 50 &             141 &                 0 &              0 &    0 &          0 &              50 &          141 &     50 &    141 \\
    gka_1-to &                 50 &              73 &                17 &              0 &    0 &         11 &              33 &           58 &     50 &     73 \\
   gka_10-ba &                 30 &             225 &                 2 &              0 &    6 &          0 &              22 &           85 &     30 &    225 \\
   gka_10-to &                 30 &             423 &                 0 &              0 &   19 &          0 &              11 &           48 &     30 &    423 \\
   gka_11-ba &                 40 &             400 &                 1 &              0 &    7 &          2 &              32 &          180 &     40 &    400 \\
   gka_11-to &                 40 &             765 &                 0 &              0 &   29 &          0 &              11 &           48 &     40 &    765 \\
   gka_12-ba &                 50 &             625 &                 0 &              0 &    6 &          0 &              44 &          381 &     50 &    625 \\
   gka_12-to &                 50 &            1202 &                 0 &              0 &   35 &          0 &              15 &           96 &     50 &   1202 \\
   gka_13-ba &                 60 &             900 &                 0 &              0 &    4 &          0 &              56 &          686 &     60 &    900 \\
   gka_13-to &                 60 &            1745 &                 0 &              0 &   43 &          0 &              17 &          126 &     60 &   1745 \\
   gka_14-ba &                 70 &            1225 &                 0 &              0 &    5 &          0 &              65 &          912 &     70 &   1225 \\
   gka_14-to &                 70 &            2380 &                 5 &              0 &   65 &          0 &               0 &            0 &     70 &   2380 \\
   gka_15-ba &                 80 &            1600 &                 1 &              0 &    8 &          0 &              71 &         1056 &     80 &   1600 \\
   gka_15-to &                 80 &            3111 &                 5 &              0 &   75 &          0 &               0 &            0 &     80 &   3111 \\
   gka_16-ba &                 90 &            2025 &                 0 &              0 &    4 &          0 &              86 &         1691 &     90 &   2025 \\
   gka_16-to &                 90 &            3953 &                 0 &              0 &   80 &          0 &              10 &           37 &     90 &   3953 \\
   gka_17-ba &                100 &            2500 &                 0 &              0 &    3 &          0 &              97 &         2219 &    100 &   2500 \\
   gka_17-to &                100 &            4892 &                 0 &              0 &   93 &          1 &               7 &           16 &    100 &   4892 \\
   gka_18-ba &                125 &            3906 &                 0 &              0 &    4 &          0 &             121 &         3451 &    125 &   3906 \\
   gka_18-to &                125 &            7657 &                 5 &              0 &  120 &          0 &               0 &            0 &    125 &   7657 \\
   gka_19-ba &                 40 &             384 &                 0 &              0 &    3 &          0 &              37 &          284 &     40 &    384 \\
   gka_19-to &                 40 &             615 &                 0 &              0 &    0 &          0 &              40 &          615 &     40 &    615 \\
    gka_2-ba &                 60 &             171 &                 0 &              0 &    0 &          0 &              60 &          171 &     60 &    171 \\
    gka_2-to &                 60 &             115 &                10 &              0 &    1 &          7 &              49 &          100 &     60 &    115 \\
   gka_20-ba &                 50 &             544 &                 0 &              0 &    1 &          0 &              49 &          503 &     50 &    544 \\
   gka_20-to &                 50 &             734 &                 0 &              0 &    0 &          0 &              50 &          734 &     50 &    734 \\
   gka_21-ba &                 60 &             576 &                 1 &              0 &    2 &          0 &              57 &          488 &     60 &    576 \\
   gka_21-to &                 60 &             637 &                 0 &              0 &    0 &          0 &              60 &          637 &     60 &    637 \\
   gka_22-ba &                 70 &             649 &                 0 &              0 &    0 &          0 &              70 &          649 &     70 &    649 \\
   gka_22-to &                 70 &             635 &                 0 &              0 &    0 &          0 &              70 &          635 &     70 &    635 \\
   gka_23-ba &                 80 &             639 &                 0 &              0 &    0 &          0 &              80 &          639 &     80 &    639 \\
   gka_23-to &                 80 &             561 &                 0 &              0 &    0 &          0 &              80 &          561 &     80 &    561 \\
   gka_24-ba &                 90 &             425 &                 0 &              0 &    0 &          0 &              90 &          425 &     90 &    425 \\
   gka_24-to &                 90 &             301 &                 1 &              0 &    0 &          0 &              89 &          300 &     90 &    301 \\
   gka_25-ba &                100 &             475 &                 0 &              0 &    0 &          0 &             100 &          475 &    100 &    475 \\
   gka_25-to &                100 &             407 &                 1 &              0 &    0 &          0 &              99 &          406 &    100 &    407 \\
   gka_26-ba &                100 &             475 &                 0 &              0 &    0 &          0 &             100 &          475 &    100 &    475 \\
   gka_26-to &                100 &             396 &                 0 &              0 &    0 &          0 &             100 &          396 &    100 &    396 \\
   gka_27-ba &                100 &             979 &                 0 &              0 &    0 &          0 &             100 &          979 &    100 &    979 \\
   gka_27-to &                100 &             919 &                 0 &              0 &    0 &          0 &             100 &          919 &    100 &    919 \\
   gka_28-ba &                100 &            1275 &                 1 &              0 &    0 &          0 &              99 &         1274 &    100 &   1275 \\
   gka_28-to &                100 &            1358 &                 0 &              0 &    0 &          0 &             100 &         1358 &    100 &   1358 \\
   gka_29-ba &                100 &            1600 &                 0 &              0 &    0 &          0 &             100 &         1600 &    100 &   1600 \\
   gka_29-to &                100 &            1950 &                 0 &              0 &    0 &          0 &             100 &         1950 &    100 &   1950 \\
    gka_3-ba &                 70 &             264 &                 0 &              0 &    0 &          0 &              70 &          264 &     70 &    264 \\
    gka_3-to &                 70 &             166 &                 2 &              0 &    0 &          7 &              68 &          165 &     70 &    166 \\
   gka_30-ba &                100 &            1875 &                 0 &              0 &    0 &          0 &             100 &         1875 &    100 &   1875 \\
   gka_30-to &                100 &            2348 &                 0 &              0 &    0 &          0 &             100 &         2348 &    100 &   2348 \\
   gka_31-ba &                100 &            2100 &                 0 &              0 &    0 &          0 &             100 &         2100 &    100 &   2100 \\
   gka_31-to &                100 &            2910 &                 0 &              0 &    0 &          0 &             100 &         2910 &    100 &   2910 \\
   gka_32-ba &                100 &            2275 &                 0 &              0 &    0 &          0 &             100 &         2275 &    100 &   2275 \\
   gka_32-to &                100 &            3425 &                 0 &              0 &    0 &          0 &             100 &         3425 &    100 &   3425 \\
   gka_33-ba &                100 &            2400 &                 0 &              0 &    4 &          0 &              96 &         2055 &    100 &   2400 \\
   gka_33-to &                100 &            3913 &                 0 &              0 &    0 &          0 &             100 &         3913 &    100 &   3913 \\
   gka_34-ba &                100 &            2464 &                 0 &              0 &    1 &          0 &              99 &         2369 &    100 &   2464 \\
   gka_34-to &                100 &            4376 &                 0 &              0 &    0 &          0 &             100 &         4376 &    100 &   4376 \\
   gka_35-ba &                100 &            2499 &                 0 &              0 &    6 &          0 &              94 &         1959 &    100 &   2499 \\
   gka_35-to &                100 &            4886 &                 0 &              0 &   90 &          0 &              10 &           36 &    100 &   4886 \\
    gka_4-ba &                 80 &             304 &                 0 &              0 &    0 &          0 &              80 &          304 &     80 &    304 \\
    gka_4-to &                 80 &             234 &                 4 &              0 &    0 &          3 &              76 &          230 &     80 &    234 \\
    gka_5-ba &                 50 &             225 &                 0 &              0 &    0 &          0 &              50 &          225 &     50 &    225 \\
    gka_5-to &                 50 &             180 &                 0 &              0 &    0 &          0 &              50 &          180 &     50 &    180 \\
    gka_6-ba &                 30 &             144 &                 0 &              0 &    0 &          0 &              30 &          144 &     30 &    144 \\
    gka_6-to &                 30 &             159 &                 0 &              0 &    0 &          0 &              30 &          159 &     30 &    159 \\
    gka_7-ba &                 30 &             176 &                 2 &              0 &    2 &          0 &              26 &          133 &     30 &    176 \\
    gka_7-to &                 30 &             196 &                 0 &              0 &    0 &          0 &              30 &          196 &     30 &    196 \\
    gka_8-ba &                100 &             384 &                 0 &              0 &    0 &          0 &             100 &          384 &    100 &    384 \\
    gka_8-to &                100 &             214 &                 8 &              0 &    0 &          9 &              92 &          206 &    100 &    214 \\
    gka_9-ba &                 20 &             100 &                 5 &              0 &    6 &          3 &               9 &           15 &     20 &    100 \\
    gka_9-to &                 20 &             183 &                 5 &              0 &   15 &          0 &               0 &            0 &     20 &    183 \\
      j10-ba &                 57 &             162 &                 0 &              0 &    0 &          0 &              57 &          162 &     57 &    162 \\
      j10-to &                 57 &              66 &                28 &              0 &    0 &          9 &              30 &           47 &     57 &     66 \\
      j11-ba &                 51 &             230 &                 0 &              0 &    0 &          0 &              51 &          230 &     51 &    230 \\
      j11-to &                 51 &             125 &                 4 &              0 &    0 &          4 &              47 &          121 &     51 &    125 \\
      j13-ba &                 78 &             225 &                10 &              0 &    4 &         11 &              64 &          139 &     78 &    225 \\
      j13-to &                 78 &             116 &                23 &              0 &    0 &         16 &              56 &           95 &     78 &    116 \\
      j14-ba &                 72 &             140 &                64 &              0 &    9 &          0 &               0 &            0 &     72 &    140 \\
      j14-to &                 72 &              49 &                71 &              0 &    1 &          0 &               0 &            0 &     72 &     49 \\
      j15-ba &                 45 &              86 &                42 &              0 &    5 &          0 &               0 &            0 &     45 &     86 \\
      j15-to &                 45 &              25 &                45 &              0 &    0 &          0 &               0 &            0 &     45 &     25 \\
      j16-ba &                 14 &              13 &                14 &              0 &    0 &          0 &               0 &            0 &     14 &     13 \\
      j16-to &                 14 &               8 &                14 &              0 &    0 &          0 &               0 &            0 &     14 &      8 \\
      j17-ba &                 81 &             308 &                 0 &              0 &    0 &          0 &              81 &          308 &     81 &    308 \\
      j17-to &                 81 &             197 &                 5 &              0 &    0 &          5 &              76 &          193 &     81 &    197 \\
      j18-ba &                 73 &             340 &                 0 &              0 &    0 &          0 &              73 &          340 &     73 &    340 \\
      j18-to &                 73 &             174 &                 6 &              0 &    1 &         10 &              66 &          160 &     73 &    174 \\
      j19-ba &                101 &             198 &                45 &              0 &    5 &         22 &              51 &           81 &    101 &    198 \\
      j19-to &                101 &              93 &                70 &              0 &    0 &         12 &              32 &           44 &    101 &     93 \\
      j20-ba &                241 &             714 &                 0 &              0 &    0 &          0 &             241 &          714 &    241 &    714 \\
      j20-to &                241 &             317 &               241 &              0 &    0 &          0 &               0 &            0 &    241 &    317 \\
      j21-ba &                 33 &             116 &                 2 &              0 &    2 &          0 &              29 &           86 &     33 &    116 \\
      j21-to &                 33 &              70 &                 2 &              0 &    0 &          1 &              31 &           68 &     33 &     70 \\
      j22-ba &                 76 &             420 &                 0 &              0 &    0 &          0 &              76 &          420 &     76 &    420 \\
      j22-to &                 76 &             226 &                 3 &              0 &    0 &          3 &              73 &          225 &     76 &    226 \\
      j23-ba &                 76 &             355 &                 0 &              0 &    0 &          0 &              76 &          355 &     76 &    355 \\
      j23-to &                 76 &             265 &                 0 &              0 &    0 &          1 &              76 &          265 &     76 &    265 \\
      j24-ba &                150 &             441 &                 0 &              0 &    0 &          0 &             150 &          441 &    150 &    441 \\
      j24-to &                150 &             197 &                63 &              0 &    0 &         28 &              89 &          143 &    150 &    197 \\
      j25-ba &                 14 &              13 &                14 &              0 &    0 &          0 &               0 &            0 &     14 &     13 \\
      j25-to &                 14 &               8 &                14 &              0 &    0 &          0 &               0 &            0 &     14 &      8 \\
      j26-ba &                 65 &             186 &                 0 &              0 &    0 &          0 &              65 &          186 &     65 &    186 \\
      j26-to &                 65 &              89 &                28 &              0 &    0 &         10 &              38 &           65 &     65 &     89 \\
      j28-ba &                 96 &             540 &                 0 &              0 &    0 &          0 &              96 &          540 &     96 &    540 \\
      j28-to &                 96 &             325 &                 2 &              0 &    0 &          2 &              94 &          324 &     96 &    325 \\
\bottomrule
\end{tabular}


==> tables/heuristic_approx_factors_synthetic.tex <==
\begin{tabular}{lrcrrrcrrrcrrrcrrrl}
\toprule
\multicolumn{2}{c}{\textbf{Timeout:}} &
\multicolumn{3}{c}{\textbf{0.01(s)}} & \phantom{Q} &
\multicolumn{3}{c}{\textbf{0.1(s)}} & \phantom{Q} &
\multicolumn{3}{c}{\textbf{1(s)}} & \phantom{Q} &
\multicolumn{3}{c}{\textbf{10(s)}}\\
\cmidrule(lr){3-5}
\cmidrule(lr){7-9}
\cmidrule(lr){11-13}
\cmidrule(lr){15-17}
\textbf{Dataset} & &
\textsf{HE} & \textsf{IC} & \textsf{ILP} &  &
\textsf{HE} & \textsf{IC} & \textsf{ILP} &  &
\textsf{HE} & \textsf{IC} & \textsf{ILP} &  &
\textsf{HE} & \textsf{IC} & \textsf{ILP}\\
\midrule
\texttt{WH-aa} & &
1.38 & \textbf{1.29} & 8.05 & &
1.27 & \textbf{1.17} & 2.19 & &
1.19 & 1.12 & \checkmark & &
1.19 & 1.06 & \checkmark\\
\midrule
\texttt{aa-ER} && \textbf{1.24} & 1.29 & 1.43 && \textbf{1.14} & 1.19 & 1.43 && 1.14 & \textbf{1.12} & 1.13 && 1.14 & 1.12 & \checkmark\\
\texttt{aa-TO} && \textbf{1.95} & 2.00 & 7.33 && \textbf{1.47} & 1.53 & 3.24 && 1.47 & 1.42 & \checkmark && 1.47 & 1.32 & \checkmark\\
\texttt{aa-CL} && \textbf{1.21} & 1.25 & 1.32 && 1.19 & \textbf{1.17} & 1.22 && 1.17 & 1.12 & \checkmark && 1.14 & 1.07 & \checkmark\\
\texttt{aa-BA} && 1.39 & \textbf{1.36} & 1.60 && \textbf{1.27} & 1.29 & 1.39 && 1.23 & 1.23 & \textbf{1.09} && 1.17 & 1.18 & \textbf{1.03}\\
\midrule
\texttt{WH-j} & &
\textbf{1.11} & 1.23 & 1.60 & &
1.11 & 1.11 & \checkmark & &
\checkmark & \checkmark & \checkmark & &
\checkmark & \checkmark & \checkmark\\
\midrule
\texttt{j-ER} && 1.12 & \textbf{1.09} & 1.67 && 1.11 & \textbf{1.07} & 1.28 && 1.06 & 1.06 & \textbf{1.05} && 1.06 & 1.06 & \textbf{1.02}\\
\texttt{j-TO} && 2.00 & \textbf{1.30} & 3.33 && 1.50 & \textbf{1.05} & 1.20 && 1.25 & 1.05 & \checkmark && \checkmark & \checkmark & \checkmark\\
\texttt{j-CL} && \textbf{1.21} & 1.26 & 1.25 && 1.21 & \textbf{1.11} & 1.21 && 1.11 & 1.11 & \checkmark && 1.11 & 1.05 & \checkmark\\
\texttt{j-BA} && 1.50 & \textbf{1.32} & 1.50 && \textbf{1.24} & \textbf{1.24} & 1.28 && 1.20 & 1.16 & \textbf{1.03} && 1.20 & 1.12 & \checkmark\\
\midrule
\texttt{b-50} & &
1.11 & \textbf{1.09} & 1.56 & &
1.09 & \textbf{1.07} & 1.21 & &
1.08 & \checkmark & \checkmark & &
\checkmark & \checkmark & \checkmark\\
\midrule
\texttt{b-50-ER} && 1.14 & \textbf{1.08} & 1.71 && 1.14 & \checkmark & 1.17 && \checkmark & \checkmark & \checkmark && \checkmark & \checkmark & \checkmark\\
\texttt{b-50-TO} && 1.25 & \checkmark & 2.00 && 1.12 & \checkmark & 1.10 && \checkmark & \checkmark & \checkmark && \checkmark & \checkmark & \checkmark\\
\texttt{b-50-CL} && 1.18 & \textbf{1.10} & 1.38 && 1.09 & \checkmark & 1.17 && \checkmark & \checkmark & \checkmark && \checkmark & \checkmark & \checkmark\\
\texttt{b-50-BA} && 1.10 & \checkmark & 1.30 && \checkmark & \checkmark & \checkmark && \checkmark & \checkmark & \checkmark && \checkmark & \checkmark & \checkmark\\
\midrule
\texttt{b-100} & &
\textbf{1.10} & \textbf{1.10} & 1.17 & &
\textbf{1.07} & \textbf{1.07} & 1.17 & &
\textbf{1.05} & \textbf{1.05} & 1.10 & &
1.05 & 1.05 & \textbf{1.02}\\
\midrule
\texttt{b-100-ER} & &
1.12 & \textbf{1.10} & 1.17 & &
1.09 & \textbf{1.05} & 1.17 & &
\textbf{1.02} & \textbf{1.02} & 1.10 & &
1.05 & 1.05 & \textbf{1.02}\\
\texttt{b-100-TO} && \textbf{1.09} & 1.17 & 1.17 && \textbf{1.06} & 1.14 & 1.15 && 1.06 & 1.11 & 1.03 && 1.06 & 1.09 & \checkmark\\
\texttt{b-100-CL} && \textbf{1.13} & 1.18 & 1.18 && \textbf{1.11} & 1.12 & 1.18 && \textbf{1.08} & 1.10 & \textbf{1.08} && 1.08 & 1.10 & \textbf{1.05}\\
\texttt{b-100-BA} && \textbf{1.14} & 1.18 & 1.19 && 1.14 & \textbf{1.11} & 1.18 && 1.11 & 1.11 & \textbf{1.05} && 1.11 & 1.04 & \checkmark\\
\midrule
\texttt{gka} & &
1.21 & \textbf{1.18} & 1.34 & &
\textbf{1.18} & \textbf{1.18} & \textbf{1.18} & &
1.11 & 1.14 & \textbf{1.07} & &
1.11 & 1.14 & \textbf{1.02}\\
\midrule
\texttt{gka-ER} && \textbf{1.11} & 1.19 & 1.20 && \textbf{1.11} & \textbf{1.11} & 1.20 && 1.11 & 1.11 & \textbf{1.04} && 1.11 & 1.11 & \checkmark\\
\texttt{gka-CL} && \textbf{1.15} & \textbf{1.15} & 1.38 && \textbf{1.12} & \textbf{1.12} & 1.31 && 1.08 & 1.08 & \textbf{1.07} && 1.08 & 1.08 & \checkmark\\
\texttt{gka-BA} && \textbf{1.14} & 1.20 & 2.48 && 1.14 & \textbf{1.11} & 2.15 && 1.11 & 1.11 & \textbf{1.05} && 1.11 & 1.04 & \checkmark\\
\texttt{gka-TO} && \textbf{1.14} & 1.19 & 1.62 && 1.14 & \textbf{1.11} & 1.36 && \textbf{1.07} & 1.11 & \textbf{1.07} && 1.07 & 1.11 & \textbf{1.03}\\
\bottomrule
\end{tabular}


==> tables/ic_select.tex <==
\begin{tabular}{llrrrrrrrr}
\toprule
& & \multicolumn{7}{c}{\textbf{OCT Size}} \\
\cmidrule(lr){3-9}
\textbf{Dataset} & $p$ & \textbf{Mean} & \textbf{S.D.} & \textbf{Min} & \textbf{25\%} & \textbf{50\%} & \textbf{75\%} & \textbf{Max}\\
\midrule
\multicolumn{4}{l}{\textbf{Timeout: 1 (s)}}\\
\midrule
\texttt{aa-42}
& 0 &  51.8 &  13.4 &  33 &  42 &  49 &  59 &  85 \\
& 1 &  31.0 &   1.2 &  30 &  30 &  31 &  32 &  35 \\
& 2 &  31.9 &   0.3 &  31 &  32 &  32 &  32 &  32 \\
\texttt{gka-2}
& 0 &  16.8 &   0.9 &  16 &  16 &  17 &  17 &  19 \\
& 1 &  16.0 &   0.0 &  16 &  16 &  16 &  16 &  16 \\
& 2 &  16.0 &   0.0 &  16 &  16 &  16 &  16 &  16 \\
\midrule
\multicolumn{4}{l}{\textbf{Timeout: 10 (s)}}\\
\midrule
\texttt{aa-41}
& 0 &  67.0 &  14.4 &  48 &  55 &  64 &  75 &  110 \\
& 1 &  41.4 &   1.2 &  40 &  40 &  41 &  42 &   44 \\
& 2 &  41.2 &   0.7 &  40 &  41 &  41 &  41 &   43 \\
\texttt{gka-3}
& 0 &  25.2 &   1.6 &  23 &  24 &  25 &  26 &   29 \\
& 1 &  23.3 &   0.5 &  23 &  23 &  23 &  24 &   24 \\
& 2 &  23.4 &   0.5 &  23 &  23 &  23 &  24 &   24 \\
\bottomrule
\end{tabular}


==> tables/ilp_16gb.tex <==
\begin{tabular}{lrrrrrrr}
\toprule
\multicolumn{5}{c}{\textbf{Preprocessed Graph}} & \multicolumn{3}{c}{\textbf{Solver}}\\
\cmidrule(lr){1-5}
\cmidrule(lr){6-8}
\textbf{Dataset} &  $|V|$ &   $|E|$ &  $OPT$ &   Time (s) & $\textsf{CPLEX}_4^\textsc{VC}$ &    $\textsf{CPLEX}_1^\textsc{VC}$  & $\textsf{GLPK}_1^\textsc{VC}$\\
\midrule
  \texttt{gka-1} &   44 &    90 &    9 &    0.1 &  $1.0\times$ &   $1.0\times$ &     $3.0\times$ \\
  \texttt{aa-43} &   58 &   303 &   18 &    0.1 &  $1.0\times$ &   $1.0\times$ &   $163.0\times$ \\
  \texttt{aa-45} &   75 &   381 &   20 &    0.1 &  $1.0\times$ &   $1.0\times$ &   $389.0\times$ \\
  \texttt{gka-2} &   58 &   149 &   16 &    0.1 &  $1.0\times$ &   $4.0\times$ &   $206.0\times$ \\
  \texttt{aa-29} &  265 &  1048 &   21 &    0.1 &  $1.0\times$ &   $4.0\times$ &  $2375.0\times$ \\
  \texttt{aa-42} &  226 &  1100 &   30 &    0.3 &  $1.0\times$ &   $4.0\times$ &               - \\
  \texttt{aa-32} &  126 &   733 &   30 &    0.4 &  $1.0\times$ &   $3.0\times$ &               - \\
  \texttt{gka-3} &   70 &   223 &   23 &    0.8 &  $1.0\times$ &   $5.6\times$ &               - \\
  \texttt{aa-41} &  261 &  1585 &   40 &    0.7 &  $1.0\times$ &   $2.3\times$ &               - \\
 \texttt{gka-26} &  100 &   494 &   43 &   16.8 &  $1.0\times$ &   $3.3\times$ &               - \\
 \texttt{gka-24} &   90 &   400 &   37 &   17.8 &  $1.0\times$ &   $5.5\times$ &               - \\
 \texttt{gka-25} &  100 &   495 &   42 &   24.4 &  $1.0\times$ &   $8.2\times$ &               - \\
 \texttt{gka-29} &  100 &  2000 &   77 &   36.3 &  $1.0\times$ &  $11.7\times$ &               - \\
 \texttt{gka-27} &  100 &  1016 &   62 &  107.4 &  $1.0\times$ &   $4.1\times$ &               - \\
 \texttt{gka-28} &  100 &  1425 &   70 &  142.0 &  $1.0\times$ &   $2.7\times$ &               - \\
\bottomrule
\end{tabular}


==> tables/ilp_4mb.tex <==
\begin{tabular}{lrrrrrrr}
\toprule
\multicolumn{5}{c}{\textbf{Preprocessed Graph}} & \multicolumn{3}{c}{\textbf{Solver}}\\
\cmidrule(lr){1-5}
\cmidrule(lr){6-8}
\textbf{Dataset} &  $|V|$ &   $|E|$ &  $OPT$ &   Time (s) & $\textsf{CPLEX}_4^\textsc{VC}$ &    $\textsf{CPLEX}_1^\textsc{VC}$  & $\textsf{GLPK}_1^\textsc{VC}$\\
\midrule
  \texttt{gka-1} &   44 &    90 &    9 &    0.1 &  $1.0\times$ &   $1.0\times$ &  $3.0\times$ \\
  \texttt{aa-43} &   58 &   303 &   18 &    0.1 &  $1.0\times$ &   $1.0\times$ &            - \\
  \texttt{aa-45} &   75 &   381 &   20 &    0.1 &  $1.0\times$ &   $1.0\times$ &            - \\
  \texttt{gka-2} &   58 &   149 &   16 &    0.1 &  $1.0\times$ &   $4.0\times$ &            - \\
  \texttt{aa-29} &  265 &  1048 &   21 &    0.1 &  $1.0\times$ &   $4.0\times$ &            - \\
  \texttt{aa-42} &  226 &  1100 &   30 &    0.3 &  $1.0\times$ &   $4.0\times$ &            - \\
  \texttt{aa-32} &  126 &   733 &   30 &    0.4 &  $1.0\times$ &   $3.0\times$ &            - \\
  \texttt{gka-3} &   70 &   223 &   23 &    0.7 &  $1.0\times$ &   $6.4\times$ &            - \\
  \texttt{aa-41} &  261 &  1585 &   40 &    0.7 &  $1.0\times$ &   $2.3\times$ &            - \\
 \texttt{gka-26} &  100 &   494 &   43 &   26.1 &  $1.0\times$ &   $2.1\times$ &            - \\
 \texttt{gka-24} &   90 &   400 &   37 &   20.7 &  $1.0\times$ &   $4.9\times$ &            - \\
 \texttt{gka-25} &  100 &   495 &   42 &   35.3 &  $1.0\times$ &   $8.5\times$ &            - \\
 \texttt{gka-29} &  100 &  2000 &   77 &   44.1 &  $1.0\times$ &  $10.5\times$ &            - \\
 \texttt{gka-27} &  100 &  1016 &   62 &  139.0 &  $1.0\times$ &   $3.2\times$ &            - \\
 \texttt{gka-28} &  100 &  1425 &   70 &  317.1 &  $1.0\times$ &   $1.4\times$ &            - \\
\bottomrule
\end{tabular}


==> tables/old_preprocessed_select.tex <==
\begin{tabular}{lrrrcrrrrcrrrr}
\toprule
& \multicolumn{3}{c}{\textbf{Original Graph}} & &
\multicolumn{4}{c}{\textbf{Reductions}} & &
\multicolumn{3}{c}{\textbf{Reduced Graph}} \\
\cmidrule(lr){2-4}
\cmidrule(lr){6-9}
\cmidrule(lr){11-13}
 \textbf{Dataset} &  $|V|$ &  $|E|$ &  $OPT$ & \phantom{00} &  $|V_r|$ &  $|E_r|$ &  $|V_o|$ &  $|V_b|$ & \phantom{00} &  $|V' \cup V_b|$ &  $|E'|$ &  $OPT'$ \\
\midrule
\texttt{aa-10} &     69 &    181 &      6 &  &     10 &        0 &        0 &       30 &   &            59 &     181 &       6 \\
\texttt{aa-11} &    103 &    298 &     11 &  &     10 &        0 &        0 &       62 &   &            93 &     298 &      11 \\
\texttt{aa-16} &     14 &      0 &      0 &  &     14 &        0 &        0 &        0 &   &             0 &       0 &       0 \\
\texttt{aa-21} &     31 &      0 &      9 &  &     22 &        0 &        9 &        0 &   &             0 &       0 &       0 \\
\texttt{aa-41} &    300 &   1585 &     40 &  &     39 &        0 &        0 &      172 &   &           261 &    1585 &      40 \\
\texttt{aa-42} &    237 &   1100 &     30 &  &     11 &        0 &        0 &      137 &   &           226 &    1100 &      30 \\
    \midrule
    \texttt{j-10} &     57 &     97 &      3 & &      20 &        0 &        0 &       13 & &              37 &      97 &       3 \\
    \texttt{j-11} &     51 &    198 &      5 & &      14 &        0 &        0 &        8 & &              37 &     198 &       5 \\
    \texttt{j-15} &     45 &      0 &      1 & &      44 &        0 &        1 &        0 & &               0 &       0 &       0 \\
    \texttt{j-16} &     14 &      0 &      0 & &      14 &        0 &        0 &        0 & &               0 &       0 &       0 \\
    \midrule
    \texttt{gka-1} &     50 &     90 &     11 & &       4 &        0 &        2 &        9 & &              44 &      90 &       9 \\
    \texttt{gka-2} &     60 &    149 &     17 & &       1 &        0 &        1 &        1 & &              58 &     149 &      16 \\
   \texttt{gka-16} &     90 &      0 &     86 & &       4 &        0 &       86 &        0 & &               0 &       0 &       0 \\
   \texttt{gka-17} &    100 &      0 &     96 & &       4 &        0 &       96 &        0 & &               0 &       0 &       0 \\
   \texttt{gka-18} &    125 &     16 &    120 & &       0 &        0 &      118 &        1 & &               7 &      16 &       2 \\
   \texttt{gka-25} &    100 &    495 &     42 & &       0 &        0 &        0 &        1 & &             100 &     495 &      42 \\
    \midrule
    \texttt{b-50-1} &     50 &    108 &     11 & &       0 &        0 &        0 &        5 & &              50 &     108 &      11 \\
    \texttt{b-50-2} &     50 &    118 &     11 & &       3 &        0 &        0 &        4 & &              47 &     118 &      11 \\
   \texttt{b-100-1} &    100 &    464 &     41 & &       0 &        0 &        0 &        0 & &             100 &     464 &      41 \\
   \texttt{b-100-2} &    100 &    482 &     42 & &       0 &        0 &        0 &        0 & &             100 &     482 &      42 \\
\bottomrule
\end{tabular}


==> tables/preprocessed_full_part1.tex <==
\begin{tabular}{lrrrrrrrrrr}
\toprule
& \multicolumn{3}{c}{\textbf{Original Graph}} & \multicolumn{4}{c}{\textbf{Results}} &
\multicolumn{3}{c}{\textbf{Reduced Graph}} \\
\cmidrule(lr){2-4}
\cmidrule(lr){5-8}
\cmidrule(lr){9-11}
  \textbf{Dataset} &  $|V|$ &  $|E|$ &  $OPT$ &  $|V_r|$ &  $|E_r|$ &  $|V_o|$ &  $|V_b|$ &  $|V' \cup V_b|$ &  $|E'|$ &  $OPT'$ \\
\midrule
\texttt{aa-10} &     69 &    181 &      6 &       10 &        0 &        0 &       30 &               59 &     181 &       6 \\
\texttt{aa-11} &    103 &    298 &     11 &       10 &        0 &        0 &       62 &               93 &     298 &      11 \\
\texttt{aa-13} &    131 &    375 &     12 &       10 &        0 &        0 &       79 &              121 &     375 &      12 \\
\texttt{aa-14} &    127 &    512 &     19 &       16 &        0 &        0 &       66 &              111 &     512 &      19 \\
\texttt{aa-15} &     67 &    146 &      7 &       15 &        0 &        1 &       21 &               51 &     146 &       6 \\
\texttt{aa-16} &     14 &      0 &      0 &       14 &        0 &        0 &        0 &                0 &       0 &       0 \\
\texttt{aa-17} &    153 &    628 &     25 &        7 &        0 &        0 &       91 &              146 &     628 &      25 \\
\texttt{aa-18} &     90 &    373 &     14 &       11 &        0 &        0 &       33 &               79 &     373 &      14 \\
\texttt{aa-19} &    192 &    636 &     19 &       11 &        0 &        0 &      120 &              181 &     636 &      19 \\
\texttt{aa-20} &    225 &    760 &     19 &        7 &        0 &        0 &      161 &              218 &     760 &      19 \\
\texttt{aa-21} &     31 &      0 &      9 &       22 &        0 &        9 &        0 &                0 &       0 &       0 \\
\texttt{aa-22} &    167 &    636 &     16 &        5 &        0 &        0 &      115 &              162 &     636 &      16 \\
\texttt{aa-23} &    143 &    492 &     18 &       21 &        0 &        0 &       69 &              122 &     492 &      18 \\
\texttt{aa-24} &    261 &   1099 &     21 &       12 &        0 &        0 &      169 &              249 &    1099 &      21 \\
\texttt{aa-25} &     15 &      0 &      1 &       14 &        0 &        1 &        0 &                0 &       0 &       0 \\
\texttt{aa-26} &     95 &    255 &     13 &       21 &        0 &        1 &       33 &               73 &     255 &      12 \\
\texttt{aa-27} &    120 &    322 &     11 &       12 &        0 &        0 &       61 &              108 &     322 &      11 \\
\texttt{aa-28} &    167 &    841 &     27 &       13 &        0 &        0 &       89 &              154 &     841 &      27 \\
\texttt{aa-29} &    277 &   1048 &     21 &       12 &        0 &        0 &      197 &              265 &    1048 &      21 \\
\texttt{aa-30} &     39 &     61 &      4 &        9 &        0 &        0 &       12 &               30 &      61 &       4 \\
\texttt{aa-31} &     30 &      0 &      2 &       28 &        0 &        2 &        0 &                0 &       0 &       0 \\
\texttt{aa-32} &    151 &    733 &     30 &       25 &        0 &        0 &       61 &              126 &     733 &      30 \\
\texttt{aa-33} &    194 &    481 &      4 &       12 &        0 &        0 &      143 &              182 &     481 &       4 \\
\texttt{aa-34} &    134 &    440 &     13 &       12 &        0 &        0 &       85 &              122 &     440 &      13 \\
\texttt{aa-35} &     82 &    264 &     10 &        6 &        0 &        0 &       38 &               76 &     264 &      10 \\
\texttt{aa-36} &    112 &    309 &      7 &        9 &        0 &        0 &       68 &              103 &     309 &       7 \\
\texttt{aa-37} &     74 &    120 &      5 &       24 &        0 &        1 &       22 &               49 &     120 &       4 \\
\texttt{aa-38} &    171 &    852 &     26 &       10 &        0 &        0 &       94 &              161 &     852 &      26 \\
\texttt{aa-39} &    145 &    689 &     23 &        4 &        0 &        0 &       82 &              141 &     689 &      23 \\
\texttt{aa-40} &    140 &    604 &     22 &       20 &        0 &        0 &       60 &              120 &     604 &      22 \\
\texttt{aa-41} &    300 &   1585 &     40 &       39 &        0 &        0 &      172 &              261 &    1585 &      40 \\
\texttt{aa-42} &    237 &   1100 &     30 &       11 &        0 &        0 &      137 &              226 &    1100 &      30 \\
\texttt{aa-43} &     64 &    303 &     18 &        6 &        0 &        0 &       18 &               58 &     303 &      18 \\
\texttt{aa-44} &     60 &    157 &     10 &        7 &        0 &        0 &       23 &               53 &     157 &      10 \\
\texttt{aa-45} &     83 &    381 &     20 &        8 &        0 &        0 &       32 &               75 &     381 &      20 \\
\texttt{aa-46} &    163 &    514 &     13 &       17 &        0 &        0 &       89 &              146 &     514 &      13 \\
\texttt{aa-47} &     65 &    195 &     14 &       17 &        0 &        1 &       13 &               47 &     195 &      13 \\
\texttt{aa-48} &     90 &    330 &     17 &       14 &        0 &        0 &       35 &               76 &     330 &      17 \\
\texttt{aa-49} &     27 &      0 &      5 &       22 &        0 &        5 &        0 &                0 &       0 &       0 \\
\texttt{aa-50} &    113 &    463 &     18 &        5 &        0 &        0 &       48 &              108 &     463 &      18 \\
\texttt{aa-51} &     79 &    268 &     11 &        8 &        0 &        0 &       27 &               71 &     268 &      11 \\
\texttt{aa-52} &     68 &    183 &     14 &       20 &        0 &        2 &       14 &               46 &     183 &      12 \\
\texttt{aa-53} &     89 &    224 &     12 &        9 &        0 &        0 &       37 &               80 &     224 &      12 \\
\texttt{aa-54} &     90 &    222 &     12 &       13 &        0 &        0 &       31 &               77 &     222 &      12 \\
    \midrule
    \texttt{j-10} &     57 &     97 &      3 &       20 &        0 &        0 &       13 &               37 &      97 &       3 \\
    \texttt{j-11} &     51 &    198 &      5 &       14 &        0 &        0 &        8 &               37 &     198 &       5 \\
    \texttt{j-13} &     78 &    153 &      6 &       22 &        0 &        2 &       28 &               54 &     153 &       4 \\
    \texttt{j-14} &     72 &     55 &      4 &       52 &        0 &        1 &        3 &               19 &      55 &       3 \\
    \texttt{j-15} &     45 &      0 &      1 &       44 &        0 &        1 &        0 &                0 &       0 &       0 \\
    \texttt{j-16} &     14 &      0 &      0 &       14 &        0 &        0 &        0 &                0 &       0 &       0 \\
    \texttt{j-17} &     81 &    304 &     10 &       20 &        0 &        0 &       20 &               61 &     304 &      10 \\
    \texttt{j-18} &     73 &    284 &      9 &       15 &        0 &        0 &       11 &               58 &     284 &       9 \\
    \texttt{j-19} &    101 &    116 &      3 &       63 &        0 &        0 &       20 &               38 &     116 &       3 \\
    \texttt{j-20} &    241 &      0 &      1 &      240 &        0 &        1 &        0 &                0 &       0 &       0 \\
    \texttt{j-21} &     33 &     16 &      9 &       18 &        0 &        7 &        1 &                8 &      16 &       2 \\
    \texttt{j-22} &     76 &    384 &      9 &        9 &        0 &        0 &       23 &               67 &     384 &       9 \\
    \texttt{j-23} &     76 &    345 &     19 &       25 &        0 &        0 &        1 &               51 &     345 &      19 \\
    \texttt{j-24} &    150 &    265 &      4 &       83 &        0 &        1 &       20 &               66 &     265 &       3 \\
    \texttt{j-25} &     14 &      0 &      0 &       14 &        0 &        0 &        0 &                0 &       0 &       0 \\
    \texttt{j-26} &     66 &    126 &      6 &       29 &        0 &        0 &       10 &               37 &     126 &       6 \\
    \texttt{j-28} &     96 &    552 &     13 &       22 &        0 &        0 &       17 &               74 &     552 &      13 \\
\bottomrule
\end{tabular}


==> tables/preprocessed_full_part2.tex <==
\begin{tabular}{lrrrrrrrrrr}
\toprule
& \multicolumn{3}{c}{\textbf{Original Graph}} & \multicolumn{4}{c}{\textbf{Results}} &
\multicolumn{3}{c}{\textbf{Reduced Graph}} \\
\cmidrule(lr){2-4}
\cmidrule(lr){5-8}
\cmidrule(lr){9-11}
  \textbf{Dataset} &  $|V|$ &  $|E|$ &  $OPT$ &  $|V_r|$ &  $|E_r|$ &  $|V_o|$ &  $|V_b|$ &  $|V' \cup V_b|$ &  $|E'|$ &  $OPT'$ \\
\midrule
\texttt{b-50-1} &     50 &    108 &     11 &        0 &        0 &        0 &        5 &               50 &     108 &      11 \\
\texttt{b-50-2} &     50 &    118 &     11 &        3 &        0 &        0 &        4 &               47 &     118 &      11 \\
\texttt{b-50-3} &     50 &    132 &     14 &        0 &        0 &        0 &        3 &               50 &     132 &      14 \\
\texttt{b-50-4} &     50 &    108 &     11 &        4 &        0 &        0 &        8 &               46 &     108 &      11 \\
\texttt{b-50-5} &     50 &    131 &     13 &        0 &        0 &        0 &        3 &               50 &     131 &      13 \\
\texttt{b-50-6} &     50 &     97 &      9 &        7 &        0 &        0 &        5 &               43 &      97 &       9 \\
\texttt{b-50-7} &     50 &    116 &     10 &        1 &        0 &        1 &        4 &               48 &     116 &       9 \\
\texttt{b-50-8} &     50 &    137 &     14 &        0 &        0 &        0 &        4 &               50 &     137 &      14 \\
\texttt{b-50-9} &     50 &    118 &     12 &        4 &        0 &        0 &        2 &               46 &     118 &      12 \\
\texttt{b-50-10} &     50 &    106 &     11 &        2 &        0 &        0 &        6 &               48 &     106 &      11 \\
\midrule
\texttt{b-100-1} &    100 &    464 &     41 &        0 &        0 &        0 &        0 &              100 &     464 &      41 \\
\texttt{b-100-2} &    100 &    482 &     42 &        0 &        0 &        0 &        0 &              100 &     482 &      42 \\
\texttt{b-100-3} &    100 &    490 &     42 &        0 &        0 &        0 &        1 &              100 &     490 &      42 \\
\texttt{b-100-4} &    100 &    475 &     41 &        0 &        0 &        0 &        0 &              100 &     475 &      41 \\
\texttt{b-100-5} &    100 &    459 &     42 &        0 &        0 &        0 &        0 &              100 &     459 &      42 \\
\texttt{b-100-6} &    100 &    510 &     43 &        0 &        0 &        0 &        0 &              100 &     510 &      43 \\
\texttt{b-100-7} &    100 &    469 &     42 &        0 &        0 &        0 &        0 &              100 &     469 &      42 \\
\texttt{b-100-8} &    100 &    492 &     43 &        0 &        0 &        0 &        0 &              100 &     492 &      43 \\
\texttt{b-100-9} &    100 &    502 &     44 &        0 &        0 &        0 &        1 &              100 &     502 &      44 \\
\texttt{b-100-10} &    100 &    485 &     44 &        0 &        0 &        0 &        0 &              100 &     485 &      44 \\
\midrule
\texttt{gka-1} &     50 &     90 &     11 &        4 &        0 &        2 &        9 &               44 &      90 &       9 \\
\texttt{gka-2} &     60 &    149 &     17 &        1 &        0 &        1 &        1 &               58 &     149 &      16 \\
\texttt{gka-3} &     70 &    223 &     23 &        0 &        0 &        0 &        4 &               70 &     223 &      23 \\
\texttt{gka-4} &     80 &    304 &     28 &        0 &        0 &        0 &        0 &               80 &     304 &      28 \\
\texttt{gka-10} &     30 &     60 &     26 &        0 &        0 &       18 &        0 &               12 &      60 &       8 \\
\texttt{gka-11} &     40 &     84 &     36 &        0 &        0 &       26 &        0 &               14 &      84 &      10 \\
\texttt{gka-12} &     50 &    264 &     46 &        0 &        0 &       26 &        0 &               24 &     264 &      20 \\
\texttt{gka-13} &     60 &    180 &     56 &        0 &        0 &       40 &        0 &               20 &     180 &      16 \\
\texttt{gka-14} &     70 &    312 &     66 &        0 &        0 &       44 &        0 &               26 &     312 &      22 \\
\texttt{gka-15} &     80 &      0 &     76 &        4 &        0 &       76 &        0 &                0 &       0 &       0 \\
\texttt{gka-16} &     90 &      0 &     86 &        4 &        0 &       86 &        0 &                0 &       0 &       0 \\
\texttt{gka-17} &    100 &      0 &     96 &        4 &        0 &       96 &        0 &                0 &       0 &       0 \\
\texttt{gka-18} &    125 &     16 &    120 &        0 &        0 &      118 &        1 &                7 &      16 &       2 \\
\texttt{gka-19} &     40 &    588 &     32 &        0 &        0 &        1 &        0 &               39 &     588 &      31 \\
\texttt{gka-20} &     50 &    763 &     39 &        0 &        0 &        0 &        0 &               50 &     763 &      39 \\
\texttt{gka-21} &     60 &    701 &     40 &        0 &        0 &        0 &        0 &               60 &     701 &      40 \\
\texttt{gka-22} &     70 &    720 &     43 &        0 &        0 &        0 &        0 &               70 &     720 &      43 \\
\texttt{gka-23} &     80 &    641 &     46 &        0 &        0 &        0 &        0 &               80 &     641 &      46 \\
\texttt{gka-24} &     90 &    400 &     37 &        0 &        0 &        0 &        0 &               90 &     400 &      37 \\
\texttt{gka-25} &    100 &    495 &     42 &        0 &        0 &        0 &        1 &              100 &     495 &      42 \\
\texttt{gka-26} &    100 &    494 &     43 &        0 &        0 &        0 &        0 &              100 &     494 &      43 \\
\texttt{gka-27} &    100 &   1016 &     62 &        0 &        0 &        0 &        0 &              100 &    1016 &      62 \\
\texttt{gka-28} &    100 &   1425 &     70 &        0 &        0 &        0 &        0 &              100 &    1425 &      70 \\
\texttt{gka-29} &    100 &   2000 &     77 &        0 &        0 &        0 &        0 &              100 &    2000 &      77 \\
\texttt{gka-30} &    100 &   2414 &     82 &        0 &        0 &        0 &        0 &              100 &    2414 &      82 \\
\texttt{gka-31} &    100 &   2948 &     85 &        0 &        0 &        0 &        0 &              100 &    2948 &      85 \\
\texttt{gka-32} &    100 &   3434 &     88 &        0 &        0 &        0 &        0 &              100 &    3434 &      88 \\
\texttt{gka-33} &    100 &   3907 &     90 &        0 &        0 &        0 &        0 &              100 &    3907 &      90 \\
\texttt{gka-34} &    100 &   4346 &     92 &        0 &        0 &        0 &        0 &              100 &    4346 &      92 \\
\texttt{gka-35} &    100 &      0 &     96 &        4 &        0 &       96 &        0 &                0 &       0 &       0 \\
\bottomrule
\end{tabular}

